Operating binary strings using gliders and eaters in reaction-diffusion cellular automaton

We study transformations of 2-, 4- and 6-bit numbers in interactions between traveling and stationary localizations in the Spiral Rule reaction-diffusion cellular automaton. The Spiral Rule automaton is a hexagonal ternary-state two-dimensional cellular automaton -- a finite-state machine imitation of an activator-inhibitor reaction-diffusion system. The activator is self-inhibited in certain concentrations. The inhibitor dissociates in the absence of the activator. The Spiral Rule cellular automaton has rich spatio-temporal dynamics of traveling (glider) and stationary (eater) patterns. When a glider brushes an eater the eater may slightly change its configuration, which is updated once more every next hit. We encode binary strings in the states of eaters and sequences of gliders. We study what types of binary compositions of binary strings are implementable by sequences of gliders brushing an eater. The models developed will be used in future laboratory designs of reaction-diffusion chemical computers.

==> 6-bit-coding/0631.tex <==
\begin{picture}(40.0,75.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(4.0,67.5){\circle*{1.}}
\put(12.0,67.5){\circle*{1.}}
\put(20.0,67.5){\circle*{1.}}
\put(28.0,67.5){\circle*{1.}}
\put(36.0,67.5){\circle*{1.}}
\put(8.0,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(24.0,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(40.0,60.0){\circle*{1.}}
\put(4.0,52.5){\circle*{1.}}
\put(12.0,52.5){\circle*{1.}}
\put(20.0,52.5){\circle{7.5}}
\put(28.0,52.5){\circle{7.5}}
\put(36.0,52.5){\circle*{1.}}
\put(8.0,45.0){\circle{7.5}}
\put(16.0,45.0){\circle*{7.0}}
\put(24.0,45.0){\circle*{7.0}}
\put(32.0,45.0){\circle{7.5}}
\put(40.0,45.0){\circle*{1.}}
\put(4.0,37.5){\circle*{1.}}
\put(12.0,37.5){\circle*{7.0}}
\put(20.0,37.5){\circle{7.5}}
\put(28.0,37.5){\circle*{7.0}}
\put(36.0,37.5){\circle*{1.}}
\put(8.0,30.0){\circle{7.5}}
\put(16.0,30.0){\circle*{7.0}}
\put(24.0,30.0){\circle*{7.0}}
\put(32.0,30.0){\circle{7.5}}
\put(40.0,30.0){\circle*{1.}}
\put(4.0,22.5){\circle*{1.}}
\put(12.0,22.5){\circle{7.5}}
\put(20.0,22.5){\circle{7.5}}
\put(28.0,22.5){\circle{7.5}}
\put(36.0,22.5){\circle*{1.}}
\put(8.0,15.0){\circle*{1.}}
\put(16.0,15.0){\circle*{1.}}
\put(24.0,15.0){\circle*{1.}}
\put(32.0,15.0){\circle*{1.}}
\put(40.0,15.0){\circle*{1.}}
\put(4.0,7.5){\circle*{1.}}
\put(12.0,7.5){\circle*{1.}}
\put(20.0,7.5){\circle*{1.}}
\put(28.0,7.5){\circle*{1.}}
\put(36.0,7.5){\circle*{1.}}
\put(8.0,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(24.0,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\put(40.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}



















































































































































==> 6-bit-coding/26667.tex <==
\begin{picture}(40.0,75.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(4.0,67.5){\circle*{1.}}
\put(12.0,67.5){\circle*{1.}}
\put(20.0,67.5){\circle*{1.}}
\put(28.0,67.5){\circle*{1.}}
\put(36.0,67.5){\circle*{1.}}
\put(8.0,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(24.0,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(40.0,60.0){\circle*{1.}}
\put(4.0,52.5){\circle*{1.}}
\put(12.0,52.5){\circle{7.5}}
\put(20.0,52.5){\circle{7.5}}
\put(28.0,52.5){\circle*{1.}}
\put(36.0,52.5){\circle*{1.}}
\put(8.0,45.0){\circle{7.5}}
\put(16.0,45.0){\circle*{7.0}}
\put(24.0,45.0){\circle*{7.0}}
\put(32.0,45.0){\circle{7.5}}
\put(40.0,45.0){\circle*{1.}}
\put(4.0,37.5){\circle*{1.}}
\put(12.0,37.5){\circle*{7.0}}
\put(20.0,37.5){\circle{7.5}}
\put(28.0,37.5){\circle*{7.0}}
\put(36.0,37.5){\circle*{1.}}
\put(8.0,30.0){\circle{7.5}}
\put(16.0,30.0){\circle*{7.0}}
\put(24.0,30.0){\circle*{7.0}}
\put(32.0,30.0){\circle{7.5}}
\put(40.0,30.0){\circle*{1.}}
\put(4.0,22.5){\circle*{1.}}
\put(12.0,22.5){\circle{7.5}}
\put(20.0,22.5){\circle{7.5}}
\put(28.0,22.5){\circle{7.5}}
\put(36.0,22.5){\circle*{1.}}
\put(8.0,15.0){\circle*{1.}}
\put(16.0,15.0){\circle*{1.}}
\put(24.0,15.0){\circle*{1.}}
\put(32.0,15.0){\circle*{1.}}
\put(40.0,15.0){\circle*{1.}}
\put(4.0,7.5){\circle*{1.}}
\put(12.0,7.5){\circle*{1.}}
\put(20.0,7.5){\circle*{1.}}
\put(28.0,7.5){\circle*{1.}}
\put(36.0,7.5){\circle*{1.}}
\put(8.0,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(24.0,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\put(40.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}



















































































































































==> eater-coding/0702.tex <==
\begin{picture}(200.0,75.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(4.0,67.5){\circle*{1.}}
\put(12.0,67.5){\circle*{1.}}
\put(20.0,67.5){\circle*{1.}}
\put(28.0,67.5){\circle*{1.}}
\put(36.0,67.5){\circle*{1.}}
\put(44.0,67.5){\circle*{1.}}
\put(52.0,67.5){\circle*{1.}}
\put(60.0,67.5){\circle*{1.}}
\put(68.0,67.5){\circle*{1.}}
\put(76.0,67.5){\circle*{1.}}
\put(84.0,67.5){\circle*{1.}}
\put(92.0,67.5){\circle*{1.}}
\put(100.0,67.5){\circle*{1.}}
\put(108.0,67.5){\circle*{1.}}
\put(116.0,67.5){\circle*{1.}}
\put(124.0,67.5){\circle*{1.}}
\put(132.0,67.5){\circle*{1.}}
\put(140.0,67.5){\circle*{1.}}
\put(148.0,67.5){\circle*{1.}}
\put(156.0,67.5){\circle*{1.}}
\put(164.0,67.5){\circle*{1.}}
\put(172.0,67.5){\circle*{1.}}
\put(180.0,67.5){\circle*{1.}}
\put(188.0,67.5){\circle*{1.}}
\put(196.0,67.5){\circle*{1.}}
\put(8.0,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(24.0,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(40.0,60.0){\circle*{1.}}
\put(48.0,60.0){\circle*{1.}}
\put(56.0,60.0){\circle*{1.}}
\put(64.0,60.0){\circle*{1.}}
\put(72.0,60.0){\circle*{1.}}
\put(80.0,60.0){\circle*{1.}}
\put(88.0,60.0){\circle*{1.}}
\put(96.0,60.0){\circle*{1.}}
\put(104.0,60.0){\circle*{1.}}
\put(112.0,60.0){\circle*{1.}}
\put(120.0,60.0){\circle*{1.}}
\put(128.0,60.0){\circle*{1.}}
\put(136.0,60.0){\circle*{1.}}
\put(144.0,60.0){\circle*{1.}}
\put(152.0,60.0){\circle*{1.}}
\put(160.0,60.0){\circle*{1.}}
\put(168.0,60.0){\circle*{1.}}
\put(176.0,60.0){\circle*{1.}}
\put(184.0,60.0){\circle*{1.}}
\put(192.0,60.0){\circle*{1.}}
\put(200.0,60.0){\circle*{1.}}
\put(4.0,52.5){\circle*{1.}}
\put(12.0,52.5){\circle*{1.}}
\put(20.0,52.5){\circle{7.5}}
\put(28.0,52.5){\circle*{1.}}
\put(36.0,52.5){\circle*{1.}}
\put(44.0,52.5){\circle*{1.}}
\put(52.0,52.5){\circle*{1.}}
\put(60.0,52.5){\circle{7.5}}
\put(68.0,52.5){\circle{7.5}}
\put(76.0,52.5){\circle*{1.}}
\put(84.0,52.5){\circle*{1.}}
\put(92.0,52.5){\circle{7.5}}
\put(100.0,52.5){\circle{7.5}}
\put(108.0,52.5){\circle*{1.}}
\put(116.0,52.5){\circle*{1.}}
\put(124.0,52.5){\circle*{1.}}
\put(132.0,52.5){\circle{7.5}}
\put(140.0,52.5){\circle{7.5}}
\put(148.0,52.5){\circle{7.5}}
\put(156.0,52.5){\circle*{1.}}
\put(164.0,52.5){\circle*{1.}}
\put(172.0,52.5){\circle*{1.}}
\put(180.0,52.5){\circle*{1.}}
\put(188.0,52.5){\circle*{1.}}
\put(196.0,52.5){\circle*{1.}}
\put(8.0,45.0){\circle{7.5}}
\put(16.0,45.0){\circle*{7.0}}
\put(24.0,45.0){\circle*{7.0}}
\put(32.0,45.0){\circle{7.5}}
\put(40.0,45.0){\circle*{1.}}
\put(48.0,45.0){\circle{7.5}}
\put(56.0,45.0){\circle*{7.0}}
\put(64.0,45.0){\circle*{7.0}}
\put(72.0,45.0){\circle{7.5}}
\put(80.0,45.0){\circle*{1.}}
\put(88.0,45.0){\circle{7.5}}
\put(96.0,45.0){\circle*{7.0}}
\put(104.0,45.0){\circle*{7.0}}
\put(112.0,45.0){\circle{7.5}}
\put(120.0,45.0){\circle*{1.}}
\put(128.0,45.0){\circle{7.5}}
\put(136.0,45.0){\circle*{7.0}}
\put(144.0,45.0){\circle*{7.0}}
\put(152.0,45.0){\circle{7.5}}
\put(160.0,45.0){\circle*{1.}}
\put(168.0,45.0){\circle*{1.}}
\put(176.0,45.0){\circle*{1.}}
\put(184.0,45.0){\circle*{1.}}
\put(192.0,45.0){\circle*{1.}}
\put(200.0,45.0){\circle*{1.}}
\put(4.0,37.5){\circle*{1.}}
\put(12.0,37.5){\circle*{7.0}}
\put(20.0,37.5){\circle{7.5}}
\put(28.0,37.5){\circle*{7.0}}
\put(36.0,37.5){\circle*{1.}}
\put(44.0,37.5){\circle*{1.}}
\put(52.0,37.5){\circle*{7.0}}
\put(60.0,37.5){\circle{7.5}}
\put(68.0,37.5){\circle*{7.0}}
\put(76.0,37.5){\circle*{1.}}
\put(84.0,37.5){\circle*{1.}}
\put(92.0,37.5){\circle*{7.0}}
\put(100.0,37.5){\circle{7.5}}
\put(108.0,37.5){\circle*{7.0}}
\put(116.0,37.5){\circle*{1.}}
\put(124.0,37.5){\circle*{1.}}
\put(132.0,37.5){\circle*{7.0}}
\put(140.0,37.5){\circle{7.5}}
\put(148.0,37.5){\circle*{7.0}}
\put(156.0,37.5){\circle*{1.}}
\put(164.0,37.5){\circle*{1.}}
\put(172.0,37.5){\circle*{1.}}
\put(180.0,37.5){\circle*{1.}}
\put(188.0,37.5){\circle*{1.}}
\put(196.0,37.5){\circle*{1.}}
\put(8.0,30.0){\circle{7.5}}
\put(16.0,30.0){\circle*{7.0}}
\put(24.0,30.0){\circle*{7.0}}
\put(32.0,30.0){\circle{7.5}}
\put(40.0,30.0){\circle*{1.}}
\put(48.0,30.0){\circle{7.5}}
\put(56.0,30.0){\circle*{7.0}}
\put(64.0,30.0){\circle*{7.0}}
\put(72.0,30.0){\circle{7.5}}
\put(80.0,30.0){\circle*{1.}}
\put(88.0,30.0){\circle{7.5}}
\put(96.0,30.0){\circle*{7.0}}
\put(104.0,30.0){\circle*{7.0}}
\put(112.0,30.0){\circle{7.5}}
\put(120.0,30.0){\circle*{1.}}
\put(128.0,30.0){\circle{7.5}}
\put(136.0,30.0){\circle*{7.0}}
\put(144.0,30.0){\circle*{7.0}}
\put(152.0,30.0){\circle{7.5}}
\put(160.0,30.0){\circle*{1.}}
\put(168.0,30.0){\circle*{1.}}
\put(176.0,30.0){\circle*{1.}}
\put(184.0,30.0){\circle*{1.}}
\put(192.0,30.0){\circle*{1.}}
\put(200.0,30.0){\circle*{1.}}
\put(4.0,22.5){\circle*{1.}}
\put(12.0,22.5){\circle*{1.}}
\put(20.0,22.5){\circle{7.5}}
\put(28.0,22.5){\circle*{1.}}
\put(36.0,22.5){\circle*{1.}}
\put(44.0,22.5){\circle*{1.}}
\put(52.0,22.5){\circle*{1.}}
\put(60.0,22.5){\circle{7.5}}
\put(68.0,22.5){\circle*{1.}}
\put(76.0,22.5){\circle*{1.}}
\put(84.0,22.5){\circle*{1.}}
\put(92.0,22.5){\circle*{1.}}
\put(100.0,22.5){\circle{7.5}}
\put(108.0,22.5){\circle*{1.}}
\put(116.0,22.5){\circle*{1.}}
\put(124.0,22.5){\circle*{1.}}
\put(132.0,22.5){\circle*{1.}}
\put(140.0,22.5){\circle{7.5}}
\put(148.0,22.5){\circle*{1.}}
\put(156.0,22.5){\circle*{1.}}
\put(164.0,22.5){\circle*{1.}}
\put(172.0,22.5){\circle*{1.}}
\put(180.0,22.5){\circle*{1.}}
\put(188.0,22.5){\circle*{1.}}
\put(196.0,22.5){\circle*{1.}}
\put(8.0,15.0){\circle*{1.}}
\put(16.0,15.0){\circle*{1.}}
\put(24.0,15.0){\circle*{1.}}
\put(32.0,15.0){\circle*{1.}}
\put(40.0,15.0){\circle*{1.}}
\put(48.0,15.0){\circle*{1.}}
\put(56.0,15.0){\circle*{1.}}
\put(64.0,15.0){\circle*{1.}}
\put(72.0,15.0){\circle*{1.}}
\put(80.0,15.0){\circle*{1.}}
\put(88.0,15.0){\circle*{1.}}
\put(96.0,15.0){\circle*{1.}}
\put(104.0,15.0){\circle*{1.}}
\put(112.0,15.0){\circle*{1.}}
\put(120.0,15.0){\circle*{1.}}
\put(128.0,15.0){\circle*{1.}}
\put(136.0,15.0){\circle*{1.}}
\put(144.0,15.0){\circle*{1.}}
\put(152.0,15.0){\circle*{1.}}
\put(160.0,15.0){\circle*{1.}}
\put(168.0,15.0){\circle*{1.}}
\put(176.0,15.0){\circle*{1.}}
\put(184.0,15.0){\circle*{1.}}
\put(192.0,15.0){\circle*{1.}}
\put(200.0,15.0){\circle*{1.}}
\put(4.0,7.5){\circle*{1.}}
\put(12.0,7.5){\circle*{1.}}
\put(20.0,7.5){\circle*{1.}}
\put(28.0,7.5){\circle*{1.}}
\put(36.0,7.5){\circle*{1.}}
\put(44.0,7.5){\circle*{1.}}
\put(52.0,7.5){\circle*{1.}}
\put(60.0,7.5){\circle*{1.}}
\put(68.0,7.5){\circle*{1.}}
\put(76.0,7.5){\circle*{1.}}
\put(84.0,7.5){\circle*{1.}}
\put(92.0,7.5){\circle*{1.}}
\put(100.0,7.5){\circle*{1.}}
\put(108.0,7.5){\circle*{1.}}
\put(116.0,7.5){\circle*{1.}}
\put(124.0,7.5){\circle*{1.}}
\put(132.0,7.5){\circle*{1.}}
\put(140.0,7.5){\circle*{1.}}
\put(148.0,7.5){\circle*{1.}}
\put(156.0,7.5){\circle*{1.}}
\put(164.0,7.5){\circle*{1.}}
\put(172.0,7.5){\circle*{1.}}
\put(180.0,7.5){\circle*{1.}}
\put(188.0,7.5){\circle*{1.}}
\put(196.0,7.5){\circle*{1.}}
\put(8.0,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(24.0,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\put(40.0,0.0){\circle*{1.}}
\put(48.0,0.0){\circle*{1.}}
\put(56.0,0.0){\circle*{1.}}
\put(64.0,0.0){\circle*{1.}}
\put(72.0,0.0){\circle*{1.}}
\put(80.0,0.0){\circle*{1.}}
\put(88.0,0.0){\circle*{1.}}
\put(96.0,0.0){\circle*{1.}}
\put(104.0,0.0){\circle*{1.}}
\put(112.0,0.0){\circle*{1.}}
\put(120.0,0.0){\circle*{1.}}
\put(128.0,0.0){\circle*{1.}}
\put(136.0,0.0){\circle*{1.}}
\put(144.0,0.0){\circle*{1.}}
\put(152.0,0.0){\circle*{1.}}
\put(160.0,0.0){\circle*{1.}}
\put(168.0,0.0){\circle*{1.}}
\put(176.0,0.0){\circle*{1.}}
\put(184.0,0.0){\circle*{1.}}
\put(192.0,0.0){\circle*{1.}}
\put(200.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}



























































































































































































































































































































































==> eater/0318.tex <==
\begin{picture}(40.0,75.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(4.0,67.5){\circle*{1.}}
\put(12.0,67.5){\circle*{1.}}
\put(20.0,67.5){\circle*{1.}}
\put(28.0,67.5){\circle*{1.}}
\put(36.0,67.5){\circle*{1.}}
\put(8.0,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(24.0,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(40.0,60.0){\circle*{1.}}
\put(4.0,52.5){\circle*{1.}}
\put(12.0,52.5){\circle*{1.}}
\put(20.0,52.5){\circle{8.5}}
\put(28.0,52.5){\circle*{1.}}
\put(36.0,52.5){\circle*{1.}}
\put(8.0,45.0){\circle{8.5}}
\put(16.0,45.0){\circle*{8.5}}
\put(24.0,45.0){\circle*{8.5}}
\put(32.0,45.0){\circle{8.5}}
\put(40.0,45.0){\circle*{1.}}
\put(4.0,37.5){\circle*{1.}}
\put(12.0,37.5){\circle*{8.5}}
\put(20.0,37.5){\circle{8.5}}
\put(28.0,37.5){\circle*{8.5}}
\put(36.0,37.5){\circle*{1.}}
\put(8.0,30.0){\circle{8.5}}
\put(16.0,30.0){\circle*{8.5}}
\put(24.0,30.0){\circle*{8.5}}
\put(32.0,30.0){\circle{8.5}}
\put(40.0,30.0){\circle*{1.}}
\put(4.0,22.5){\circle*{1.}}
\put(12.0,22.5){\circle*{1.}}
\put(20.0,22.5){\circle{8.5}}
\put(28.0,22.5){\circle*{1.}}
\put(36.0,22.5){\circle*{1.}}
\put(8.0,15.0){\circle*{1.}}
\put(16.0,15.0){\circle*{1.}}
\put(24.0,15.0){\circle*{1.}}
\put(32.0,15.0){\circle*{1.}}
\put(40.0,15.0){\circle*{1.}}
\put(4.0,7.5){\circle*{1.}}
\put(12.0,7.5){\circle*{1.}}
\put(20.0,7.5){\circle*{1.}}
\put(28.0,7.5){\circle*{1.}}
\put(36.0,7.5){\circle*{1.}}
\put(8.0,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(24.0,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\put(40.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}



















































































































































==> matrices/FDistT.tex <==
\begin{scriptsize}
$$
D = \left(
\begin{smallmatrix}
3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & 2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & \\
3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & 2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & \\
3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & 1 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & \\
3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & 1 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & \\
1 & 3 & 3 & 2 & 3 & 1 & 2 & 3 & 3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & \\
1 & 3 & 3 & 2 & 3 & 1 & 2 & 3 & 3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & \\
2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & \\
2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & \\
2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & \\
2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & \\
1 & 3 & 3 & 2 & 3 & 1 & 2 & 3 & 3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & \\
1 & 3 & 3 & 2 & 3 & 1 & 2 & 3 & 3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & \\
3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & 1 & 3 & 3 & 2 & 2 & 1 & 2 & 3 & \\
3 & 2 & 1 & 3 & 2 & 3 & 3 & 1 & 1 & 3 & 3 & 2 & 1 & 2 & 2 & 3 & \\
3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & 2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & \\
3 & 2 & 2 & 1 & 2 & 3 & 1 & 2 & 2 & 1 & 3 & 2 & 1 & 2 & 2 & 3 & \\
\end{smallmatrix}
\right)
$$
\end{scriptsize}


==> matrices/matrixTEX_L1.tex <==
\begin{scriptsize}
$$\begin{smallmatrix}
\underline{0}  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &0  &\\
1  &\underline{1}  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &1  &33 &\underline{33} &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
2  &3  &\underline{2}  &\underline{3}  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &2  &3  &\\
3  &3  &\underline{3}  &\underline{3}  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &3  &35 &35 &\underline{35} &\underline{35} &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
4  &4  &6  &7  &\underline{4}  &4  &\underline{6}  &\underline{7}  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &4  &4  &6  &7  &\\
5  &5  &7  &7  &5  &\underline{5}  &\underline{7}  &\underline{7}  &5  &5  &7  &7  &5  &5  &7  &7  &5  &5  &7  &7  &5  &5  &7  &7  &5  &5  &7  &7  &5  &5  &7  &7  &37 &37 &39 &39 &37 &\underline{37} &\underline{39} &\underline{39} &37 &37 &39 &39 &37 &37 &39 &39 &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
6  &7  &6  &7  &\underline{6}  &\underline{7}  &\underline{6}  &\underline{7}  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &6  &7  &\\
7  &7  &7  &7  &\underline{7}  &\underline{7}  &\underline{7}  &\underline{7}  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &7  &39 &39 &39 &39 &\underline{39} &\underline{39} &\underline{39} &\underline{39} &39 &39 &39 &39 &39 &39 &39 &39 &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
8  &8  &8  &8  &12 &12 &14 &15 &\underline{8}  &8  &8  &8  &\underline{12} &12 &\underline{14} &\underline{15} &8  &8  &8  &8  &12 &12 &14 &15 &8  &8  &8  &8  &12 &12 &14 &15 &8  &8  &8  &8  &12 &12 &14 &15 &8  &8  &8  &8  &12 &12 &14 &15 &8  &8  &8  &8  &12 &12 &14 &15 &8  &8  &8  &8  &12 &12 &14 &15 &\\
9  &9  &9  &9  &13 &13 &15 &15 &9  &\underline{9}  &9  &9  &13 &\underline{13} &\underline{15} &\underline{15} &9  &9  &9  &9  &13 &13 &15 &15 &9  &9  &9  &9  &13 &13 &15 &15 &41 &41 &41 &41 &45 &45 &47 &47 &41 &\underline{41} &41 &41 &45 &\underline{45} &\underline{47} &\underline{47} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &\underline{10} &\underline{11} &\underline{14} &\underline{15} &\underline{14} &\underline{15} &10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &10 &11 &14 &15 &14 &15 &10 &11 &10 &11 &14 &15 &14 &15 &\\
11 &11 &11 &11 &15 &15 &15 &15 &11 &11 &\underline{11} &\underline{11} &\underline{15} &\underline{15} &\underline{15} &\underline{15} &11 &11 &11 &11 &15 &15 &15 &15 &11 &11 &11 &11 &15 &15 &15 &15 &43 &43 &43 &43 &47 &47 &47 &47 &43 &43 &\underline{43} &\underline{43} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
12 &12 &14 &15 &12 &12 &14 &15 &\underline{12} &12 &\underline{14} &\underline{15} &\underline{12} &12 &\underline{14} &\underline{15} &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &12 &12 &14 &15 &\\
13 &13 &15 &15 &13 &13 &15 &15 &13 &\underline{13} &\underline{15} &\underline{15} &13 &\underline{13} &\underline{15} &\underline{15} &13 &13 &15 &15 &13 &13 &15 &15 &13 &13 &15 &15 &13 &13 &15 &15 &45 &45 &47 &47 &45 &45 &47 &47 &45 &\underline{45} &\underline{47} &\underline{47} &45 &\underline{45} &\underline{47} &\underline{47} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
14 &15 &14 &15 &14 &15 &14 &15 &\underline{14} &\underline{15} &\underline{14} &\underline{15} &\underline{14} &\underline{15} &\underline{14} &\underline{15} &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &14 &15 &\\
15 &15 &15 &15 &15 &15 &15 &15 &\underline{15} &\underline{15} &\underline{15} &\underline{15} &\underline{15} &\underline{15} &\underline{15} &\underline{15} &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
16 &16 &16 &16 &16 &16 &16 &16 &24 &24 &24 &24 &28 &28 &30 &31 &\underline{16} &16 &16 &16 &16 &16 &16 &16 &\underline{24} &24 &24 &24 &\underline{28} &28 &\underline{30} &\underline{31} &16 &16 &16 &16 &16 &16 &16 &16 &24 &24 &24 &24 &28 &28 &30 &31 &16 &16 &16 &16 &16 &16 &16 &16 &24 &24 &24 &24 &28 &28 &30 &31 &\\
17 &17 &17 &17 &17 &17 &17 &17 &25 &25 &25 &25 &29 &29 &31 &31 &17 &\underline{17} &17 &17 &17 &17 &17 &17 &25 &\underline{25} &25 &25 &29 &\underline{29} &\underline{31} &\underline{31} &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
18 &19 &18 &19 &18 &19 &18 &19 &26 &27 &26 &27 &30 &31 &30 &31 &18 &19 &\underline{18} &\underline{19} &18 &19 &18 &19 &26 &27 &\underline{26} &\underline{27} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &18 &19 &18 &19 &18 &19 &18 &19 &26 &27 &26 &27 &30 &31 &30 &31 &18 &19 &18 &19 &18 &19 &18 &19 &26 &27 &26 &27 &30 &31 &30 &31 &\\
19 &19 &19 &19 &19 &19 &19 &19 &27 &27 &27 &27 &31 &31 &31 &31 &19 &19 &\underline{19} &\underline{19} &19 &19 &19 &19 &27 &27 &\underline{27} &\underline{27} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
20 &20 &22 &23 &20 &20 &22 &23 &28 &28 &30 &31 &28 &28 &30 &31 &20 &20 &22 &23 &\underline{20} &20 &\underline{22} &\underline{23} &\underline{28} &28 &\underline{30} &\underline{31} &\underline{28} &28 &\underline{30} &\underline{31} &20 &20 &22 &23 &20 &20 &22 &23 &28 &28 &30 &31 &28 &28 &30 &31 &20 &20 &22 &23 &20 &20 &22 &23 &28 &28 &30 &31 &28 &28 &30 &31 &\\
21 &21 &23 &23 &21 &21 &23 &23 &29 &29 &31 &31 &29 &29 &31 &31 &21 &21 &23 &23 &21 &\underline{21} &\underline{23} &\underline{23} &29 &\underline{29} &\underline{31} &\underline{31} &29 &\underline{29} &\underline{31} &\underline{31} &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
22 &23 &22 &23 &22 &23 &22 &23 &30 &31 &30 &31 &30 &31 &30 &31 &22 &23 &22 &23 &\underline{22} &\underline{23} &\underline{22} &\underline{23} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &22 &23 &22 &23 &22 &23 &22 &23 &30 &31 &30 &31 &30 &31 &30 &31 &22 &23 &22 &23 &22 &23 &22 &23 &30 &31 &30 &31 &30 &31 &30 &31 &\\
23 &23 &23 &23 &23 &23 &23 &23 &31 &31 &31 &31 &31 &31 &31 &31 &23 &23 &23 &23 &\underline{23} &\underline{23} &\underline{23} &\underline{23} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
24 &24 &24 &24 &28 &28 &30 &31 &24 &24 &24 &24 &28 &28 &30 &31 &\underline{24} &24 &24 &24 &\underline{28} &28 &\underline{30} &\underline{31} &\underline{24} &24 &24 &24 &\underline{28} &28 &\underline{30} &\underline{31} &24 &24 &24 &24 &28 &28 &30 &31 &24 &24 &24 &24 &28 &28 &30 &31 &24 &24 &24 &24 &28 &28 &30 &31 &24 &24 &24 &24 &28 &28 &30 &31 &\\
25 &25 &25 &25 &29 &29 &31 &31 &25 &25 &25 &25 &29 &29 &31 &31 &25 &\underline{25} &25 &25 &29 &\underline{29} &\underline{31} &\underline{31} &25 &\underline{25} &25 &25 &29 &\underline{29} &\underline{31} &\underline{31} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
26 &27 &26 &27 &30 &31 &30 &31 &26 &27 &26 &27 &30 &31 &30 &31 &26 &27 &\underline{26} &\underline{27} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &26 &27 &\underline{26} &\underline{27} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &26 &27 &26 &27 &30 &31 &30 &31 &26 &27 &26 &27 &30 &31 &30 &31 &26 &27 &26 &27 &30 &31 &30 &31 &26 &27 &26 &27 &30 &31 &30 &31 &\\
27 &27 &27 &27 &31 &31 &31 &31 &27 &27 &27 &27 &31 &31 &31 &31 &27 &27 &\underline{27} &\underline{27} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &27 &27 &\underline{27} &\underline{27} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &\underline{28} &28 &\underline{30} &\underline{31} &\underline{28} &28 &\underline{30} &\underline{31} &\underline{28} &28 &\underline{30} &\underline{31} &\underline{28} &28 &\underline{30} &\underline{31} &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &28 &28 &30 &31 &\\
29 &29 &31 &31 &29 &29 &31 &31 &29 &29 &31 &31 &29 &29 &31 &31 &29 &\underline{29} &\underline{31} &\underline{31} &29 &\underline{29} &\underline{31} &\underline{31} &29 &\underline{29} &\underline{31} &\underline{31} &29 &\underline{29} &\underline{31} &\underline{31} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &\\
31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &48 &48 &48 &48 &48 &48 &48 &48 &56 &56 &56 &56 &60 &60 &62 &\underline{63} &\underline{32} &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &32 &\underline{48} &48 &48 &48 &48 &48 &48 &48 &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\\
33 &\underline{33} &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &33 &\underline{33} &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &33 &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
34 &35 &34 &\underline{35} &34 &35 &34 &35 &34 &35 &34 &35 &34 &35 &34 &35 &50 &51 &50 &\underline{51} &50 &51 &50 &51 &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &34 &35 &\underline{34} &\underline{35} &34 &35 &34 &35 &34 &35 &34 &35 &34 &35 &34 &35 &50 &51 &\underline{50} &\underline{51} &50 &51 &50 &51 &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
35 &35 &35 &\underline{35} &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &51 &51 &51 &\underline{51} &51 &51 &51 &51 &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &35 &35 &\underline{35} &\underline{35} &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &35 &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
36 &36 &38 &39 &36 &36 &38 &\underline{39} &36 &36 &38 &39 &36 &36 &38 &39 &52 &52 &54 &55 &52 &52 &54 &\underline{55} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &36 &36 &38 &39 &\underline{36} &36 &\underline{38} &\underline{39} &36 &36 &38 &39 &36 &36 &38 &39 &52 &52 &54 &55 &\underline{52} &52 &\underline{54} &\underline{55} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\\
37 &37 &39 &39 &37 &\underline{37} &39 &\underline{39} &37 &37 &39 &39 &37 &37 &39 &39 &53 &53 &55 &55 &53 &\underline{53} &55 &\underline{55} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &37 &37 &39 &39 &37 &\underline{37} &\underline{39} &\underline{39} &37 &37 &39 &39 &37 &37 &39 &39 &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
38 &39 &38 &39 &38 &\underline{39} &38 &\underline{39} &38 &39 &38 &39 &38 &39 &38 &39 &54 &55 &54 &55 &54 &\underline{55} &54 &\underline{55} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &38 &39 &38 &39 &\underline{38} &\underline{39} &\underline{38} &\underline{39} &38 &39 &38 &39 &38 &39 &38 &39 &54 &55 &54 &55 &\underline{54} &\underline{55} &\underline{54} &\underline{55} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
39 &39 &39 &39 &39 &\underline{39} &39 &\underline{39} &39 &39 &39 &39 &39 &39 &39 &39 &55 &55 &55 &55 &55 &\underline{55} &55 &\underline{55} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &39 &39 &39 &39 &\underline{39} &\underline{39} &\underline{39} &\underline{39} &39 &39 &39 &39 &39 &39 &39 &39 &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
40 &40 &40 &40 &44 &44 &46 &47 &40 &40 &40 &40 &44 &44 &46 &\underline{47} &56 &56 &56 &56 &60 &60 &62 &\underline{63} &56 &56 &56 &56 &60 &60 &62 &\underline{63} &40 &40 &40 &40 &44 &44 &46 &47 &\underline{40} &40 &40 &40 &\underline{44} &44 &\underline{46} &\underline{47} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\\
41 &41 &41 &41 &45 &45 &47 &47 &41 &\underline{41} &41 &41 &45 &\underline{45} &47 &\underline{47} &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &41 &41 &41 &41 &45 &45 &47 &47 &41 &\underline{41} &41 &41 &45 &\underline{45} &\underline{47} &\underline{47} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
42 &43 &42 &43 &46 &47 &46 &47 &42 &43 &42 &\underline{43} &46 &\underline{47} &46 &\underline{47} &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &42 &43 &42 &43 &46 &47 &46 &47 &42 &43 &\underline{42} &\underline{43} &\underline{46} &\underline{47} &\underline{46} &\underline{47} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
43 &43 &43 &43 &47 &47 &47 &47 &43 &43 &43 &\underline{43} &47 &\underline{47} &47 &\underline{47} &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &43 &43 &43 &43 &47 &47 &47 &47 &43 &43 &\underline{43} &\underline{43} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
44 &44 &46 &47 &44 &44 &46 &47 &44 &44 &46 &\underline{47} &44 &44 &46 &\underline{47} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &44 &44 &46 &47 &44 &44 &46 &47 &\underline{44} &44 &\underline{46} &\underline{47} &\underline{44} &44 &\underline{46} &\underline{47} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\\
45 &45 &47 &47 &45 &45 &47 &47 &45 &\underline{45} &47 &\underline{47} &45 &\underline{45} &47 &\underline{47} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &45 &45 &47 &47 &45 &45 &47 &47 &45 &\underline{45} &\underline{47} &\underline{47} &45 &\underline{45} &\underline{47} &\underline{47} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
46 &47 &46 &47 &46 &47 &46 &47 &46 &\underline{47} &46 &\underline{47} &46 &\underline{47} &46 &\underline{47} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &46 &47 &46 &47 &46 &47 &46 &47 &\underline{46} &\underline{47} &\underline{46} &\underline{47} &\underline{46} &\underline{47} &\underline{46} &\underline{47} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
47 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{47} &47 &\underline{47} &47 &\underline{47} &47 &\underline{47} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{47} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
48 &48 &48 &48 &48 &48 &48 &48 &56 &56 &56 &56 &60 &60 &62 &\underline{63} &48 &48 &48 &48 &48 &48 &48 &48 &56 &56 &56 &56 &60 &60 &62 &\underline{63} &\underline{48} &48 &48 &48 &48 &48 &48 &48 &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\underline{48} &48 &48 &48 &48 &48 &48 &48 &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\\
49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &49 &\underline{49} &49 &49 &49 &49 &49 &49 &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
50 &51 &50 &\underline{51} &50 &51 &50 &51 &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &50 &51 &50 &\underline{51} &50 &51 &50 &51 &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &50 &51 &\underline{50} &\underline{51} &50 &51 &50 &51 &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &50 &51 &\underline{50} &\underline{51} &50 &51 &50 &51 &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
51 &51 &51 &\underline{51} &51 &51 &51 &51 &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &51 &51 &51 &\underline{51} &51 &51 &51 &51 &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{51} &\underline{51} &51 &51 &51 &51 &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
52 &52 &54 &55 &52 &52 &54 &\underline{55} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &52 &52 &54 &55 &52 &52 &54 &\underline{55} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &52 &52 &54 &55 &\underline{52} &52 &\underline{54} &\underline{55} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &52 &52 &54 &55 &\underline{52} &52 &\underline{54} &\underline{55} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\\
53 &53 &55 &55 &53 &\underline{53} &55 &\underline{55} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &53 &53 &55 &55 &53 &\underline{53} &55 &\underline{55} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &53 &53 &55 &55 &53 &\underline{53} &\underline{55} &\underline{55} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
54 &55 &54 &55 &54 &\underline{55} &54 &\underline{55} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &54 &55 &54 &55 &54 &\underline{55} &54 &\underline{55} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &54 &55 &54 &55 &\underline{54} &\underline{55} &\underline{54} &\underline{55} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &54 &55 &54 &55 &\underline{54} &\underline{55} &\underline{54} &\underline{55} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
55 &55 &55 &55 &55 &\underline{55} &55 &\underline{55} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &55 &\underline{55} &55 &\underline{55} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{55} &\underline{55} &\underline{55} &\underline{55} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
56 &56 &56 &56 &60 &60 &62 &\underline{63} &56 &56 &56 &56 &60 &60 &62 &\underline{63} &56 &56 &56 &56 &60 &60 &62 &\underline{63} &56 &56 &56 &56 &60 &60 &62 &\underline{63} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\underline{56} &56 &56 &56 &\underline{60} &60 &\underline{62} &\underline{63} &\\
57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &63 &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &57 &\underline{57} &57 &57 &61 &\underline{61} &\underline{63} &\underline{63} &\\
58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &58 &59 &58 &\underline{59} &62 &\underline{63} &62 &\underline{63} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &58 &59 &\underline{58} &\underline{59} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &59 &59 &59 &\underline{59} &63 &\underline{63} &63 &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{59} &\underline{59} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &60 &60 &62 &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\underline{60} &60 &\underline{62} &\underline{63} &\\
61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &63 &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &61 &\underline{61} &\underline{63} &\underline{63} &\\
62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\\
63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
\end{smallmatrix}$$
\end{scriptsize}


==> matrices/matrixTEX_L2.tex <==
\begin{scriptsize}
$$\begin{smallmatrix}
\underline{0}  &\underline{1}  &\underline{2}  &2  &\underline{4}  &\underline{5}  &4  &5  &\underline{8}  &\underline{9}  &\underline{10} &10 &8  &9  &10 &10 &\underline{16} &\underline{17} &\underline{18} &18 &\underline{20} &\underline{21} &20 &21 &16 &17 &18 &18 &20 &21 &20 &21 &\underline{32} &\underline{33} &\underline{34} &34 &\underline{36} &\underline{37} &36 &37 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &32 &33 &34 &34 &36 &37 &36 &37 &40 &41 &42 &42 &40 &41 &42 &42 &\\
\underline{1}  &\underline{1}  &3  &\underline{3}  &\underline{5}  &\underline{5}  &5  &5  &\underline{9}  &\underline{9}  &11 &\underline{11} &9  &9  &11 &11 &\underline{17} &\underline{17} &19 &\underline{19} &\underline{21} &\underline{21} &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &1  &1  &3  &3  &5  &5  &5  &5  &9  &9  &11 &11 &9  &9  &11 &11 &17 &17 &19 &19 &21 &21 &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &\\
\underline{2}  &2  &\underline{2}  &2  &6  &6  &\underline{6}  &6  &\underline{10} &10 &\underline{10} &10 &10 &10 &10 &10 &\underline{18} &18 &\underline{18} &18 &22 &22 &\underline{22} &22 &18 &18 &18 &18 &22 &22 &22 &22 &\underline{34} &34 &\underline{34} &34 &38 &38 &\underline{38} &38 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &34 &34 &34 &34 &38 &38 &38 &38 &42 &42 &42 &42 &42 &42 &42 &42 &\\
3  &\underline{3}  &3  &\underline{3}  &7  &7  &7  &\underline{7}  &11 &\underline{11} &11 &\underline{11} &11 &11 &11 &11 &19 &\underline{19} &19 &\underline{19} &23 &23 &23 &\underline{23} &19 &19 &19 &19 &23 &23 &23 &23 &3  &3  &3  &3  &7  &7  &7  &7  &11 &11 &11 &11 &11 &11 &11 &11 &19 &19 &19 &19 &23 &23 &23 &23 &19 &19 &19 &19 &23 &23 &23 &23 &\\
\underline{4}  &\underline{5}  &4  &5  &\underline{4}  &\underline{5}  &4  &5  &12 &13 &12 &13 &\underline{12} &\underline{13} &12 &13 &\underline{20} &\underline{21} &20 &21 &\underline{20} &\underline{21} &20 &21 &20 &21 &20 &21 &20 &21 &20 &21 &\underline{36} &\underline{37} &36 &37 &\underline{36} &\underline{37} &36 &37 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &36 &37 &36 &37 &36 &37 &36 &37 &44 &45 &44 &45 &44 &45 &44 &45 &\\
\underline{5}  &\underline{5}  &5  &5  &\underline{5}  &\underline{5}  &5  &5  &13 &13 &13 &13 &\underline{13} &\underline{13} &13 &13 &\underline{21} &\underline{21} &21 &21 &\underline{21} &\underline{21} &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &5  &5  &5  &5  &5  &5  &5  &5  &13 &13 &13 &13 &13 &13 &13 &13 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &\\
6  &6  &\underline{6}  &6  &6  &6  &\underline{6}  &6  &14 &14 &14 &14 &14 &14 &\underline{14} &14 &22 &22 &\underline{22} &22 &22 &22 &\underline{22} &22 &22 &22 &22 &22 &22 &22 &22 &22 &38 &38 &\underline{38} &38 &38 &38 &\underline{38} &38 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &38 &38 &38 &38 &38 &38 &38 &38 &46 &46 &46 &46 &46 &46 &46 &46 &\\
7  &7  &7  &\underline{7}  &7  &7  &7  &\underline{7}  &15 &15 &15 &15 &15 &15 &15 &\underline{15} &23 &23 &23 &\underline{23} &23 &23 &23 &\underline{23} &23 &23 &23 &23 &23 &23 &23 &23 &7  &7  &7  &7  &7  &7  &7  &7  &15 &15 &15 &15 &15 &15 &15 &15 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &\\
\underline{8}  &\underline{9}  &\underline{10} &10 &8  &9  &10 &10 &\underline{8}  &\underline{9}  &\underline{10} &10 &8  &9  &10 &10 &24 &25 &26 &26 &24 &25 &26 &26 &\underline{24} &\underline{25} &\underline{26} &26 &24 &25 &26 &26 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &\\
\underline{9}  &\underline{9}  &11 &\underline{11} &9  &9  &11 &11 &\underline{9}  &\underline{9}  &11 &\underline{11} &9  &9  &11 &11 &25 &25 &27 &27 &25 &25 &27 &27 &\underline{25} &\underline{25} &27 &\underline{27} &25 &25 &27 &27 &9  &9  &11 &11 &9  &9  &11 &11 &9  &9  &11 &11 &9  &9  &11 &11 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &\\
\underline{10} &10 &\underline{10} &10 &10 &10 &10 &10 &\underline{10} &10 &\underline{10} &10 &10 &10 &10 &10 &26 &26 &26 &26 &26 &26 &26 &26 &\underline{26} &26 &\underline{26} &26 &26 &26 &26 &26 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &\\
11 &\underline{11} &11 &\underline{11} &11 &11 &11 &11 &11 &\underline{11} &11 &\underline{11} &11 &11 &11 &11 &27 &27 &27 &27 &27 &27 &27 &27 &27 &\underline{27} &27 &\underline{27} &27 &27 &27 &27 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &11 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &\\
12 &13 &12 &13 &\underline{12} &\underline{13} &12 &13 &12 &13 &12 &13 &\underline{12} &\underline{13} &12 &13 &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &\underline{28} &\underline{29} &28 &29 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &\\
13 &13 &13 &13 &\underline{13} &\underline{13} &13 &13 &13 &13 &13 &13 &\underline{13} &\underline{13} &13 &13 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &\underline{29} &\underline{29} &29 &29 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &13 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &\\
14 &14 &14 &14 &14 &14 &\underline{14} &14 &14 &14 &14 &14 &14 &14 &\underline{14} &14 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &\underline{30} &30 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &\\
15 &15 &15 &15 &15 &15 &15 &\underline{15} &15 &15 &15 &15 &15 &15 &15 &\underline{15} &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{31} &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &15 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\\
\underline{16} &\underline{17} &\underline{18} &18 &\underline{20} &\underline{21} &20 &21 &16 &17 &18 &18 &20 &21 &20 &21 &\underline{16} &\underline{17} &\underline{18} &18 &\underline{20} &\underline{21} &20 &21 &16 &17 &18 &18 &20 &21 &20 &21 &48 &49 &50 &50 &52 &53 &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &\underline{48} &\underline{49} &\underline{50} &50 &\underline{52} &\underline{53} &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &\\
\underline{17} &\underline{17} &19 &\underline{19} &\underline{21} &\underline{21} &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &\underline{17} &\underline{17} &19 &\underline{19} &\underline{21} &\underline{21} &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &17 &17 &19 &19 &21 &21 &21 &21 &\\
\underline{18} &18 &\underline{18} &18 &22 &22 &\underline{22} &22 &18 &18 &18 &18 &22 &22 &22 &22 &\underline{18} &18 &\underline{18} &18 &22 &22 &\underline{22} &22 &18 &18 &18 &18 &22 &22 &22 &22 &50 &50 &50 &50 &54 &54 &54 &54 &50 &50 &50 &50 &54 &54 &54 &54 &\underline{50} &50 &\underline{50} &50 &54 &54 &\underline{54} &54 &50 &50 &50 &50 &54 &54 &54 &54 &\\
19 &\underline{19} &19 &\underline{19} &23 &23 &23 &\underline{23} &19 &19 &19 &19 &23 &23 &23 &23 &19 &\underline{19} &19 &\underline{19} &23 &23 &23 &\underline{23} &19 &19 &19 &19 &23 &23 &23 &23 &19 &19 &19 &19 &23 &23 &23 &23 &19 &19 &19 &19 &23 &23 &23 &23 &19 &19 &19 &19 &23 &23 &23 &23 &19 &19 &19 &19 &23 &23 &23 &23 &\\
\underline{20} &\underline{21} &20 &21 &\underline{20} &\underline{21} &20 &21 &20 &21 &20 &21 &20 &21 &20 &21 &\underline{20} &\underline{21} &20 &21 &\underline{20} &\underline{21} &20 &21 &20 &21 &20 &21 &20 &21 &20 &21 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &\underline{52} &\underline{53} &52 &53 &\underline{52} &\underline{53} &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &\\
\underline{21} &\underline{21} &21 &21 &\underline{21} &\underline{21} &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &\underline{21} &\underline{21} &21 &21 &\underline{21} &\underline{21} &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &21 &\\
22 &22 &\underline{22} &22 &22 &22 &\underline{22} &22 &22 &22 &22 &22 &22 &22 &22 &22 &22 &22 &\underline{22} &22 &22 &22 &\underline{22} &22 &22 &22 &22 &22 &22 &22 &22 &22 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &\underline{54} &54 &54 &54 &\underline{54} &54 &54 &54 &54 &54 &54 &54 &54 &54 &\\
23 &23 &23 &\underline{23} &23 &23 &23 &\underline{23} &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &\underline{23} &23 &23 &23 &\underline{23} &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &23 &\\
24 &25 &26 &26 &24 &25 &26 &26 &\underline{24} &\underline{25} &\underline{26} &26 &24 &25 &26 &26 &24 &25 &26 &26 &24 &25 &26 &26 &\underline{24} &\underline{25} &\underline{26} &26 &24 &25 &26 &26 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &\underline{56} &\underline{57} &\underline{58} &58 &56 &57 &58 &58 &\\
25 &25 &27 &27 &25 &25 &27 &27 &\underline{25} &\underline{25} &27 &\underline{27} &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &\underline{25} &\underline{25} &27 &\underline{27} &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &25 &25 &27 &27 &\\
26 &26 &26 &26 &26 &26 &26 &26 &\underline{26} &26 &\underline{26} &26 &26 &26 &26 &26 &26 &26 &26 &26 &26 &26 &26 &26 &\underline{26} &26 &\underline{26} &26 &26 &26 &26 &26 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &\underline{58} &58 &\underline{58} &58 &58 &58 &58 &58 &\\
27 &27 &27 &27 &27 &27 &27 &27 &27 &\underline{27} &27 &\underline{27} &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &\underline{27} &27 &\underline{27} &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &27 &\\
28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &\underline{28} &\underline{29} &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &28 &29 &\underline{28} &\underline{29} &28 &29 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &\underline{60} &\underline{61} &60 &61 &\\
29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &\underline{29} &\underline{29} &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &\underline{29} &\underline{29} &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &29 &\\
30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &\underline{30} &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &\underline{30} &30 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &\underline{62} &62 &\\
31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{31} &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{31} &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\\
\underline{32} &33 &\underline{34} &34 &\underline{36} &37 &36 &37 &\underline{40} &41 &\underline{42} &42 &40 &41 &42 &42 &32 &33 &34 &34 &36 &37 &36 &37 &40 &41 &42 &42 &40 &41 &42 &42 &\underline{32} &\underline{33} &\underline{34} &34 &\underline{36} &\underline{37} &36 &37 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &32 &33 &34 &34 &36 &37 &36 &37 &40 &41 &42 &42 &40 &41 &42 &42 &\\
\underline{33} &33 &35 &35 &\underline{37} &37 &37 &37 &\underline{41} &41 &43 &43 &41 &41 &43 &43 &33 &33 &35 &35 &37 &37 &37 &37 &41 &41 &43 &43 &41 &41 &43 &43 &\underline{33} &\underline{33} &35 &\underline{35} &\underline{37} &\underline{37} &37 &37 &\underline{41} &\underline{41} &43 &\underline{43} &41 &41 &43 &43 &33 &33 &35 &35 &37 &37 &37 &37 &41 &41 &43 &43 &41 &41 &43 &43 &\\
\underline{34} &34 &\underline{34} &34 &38 &38 &\underline{38} &38 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &34 &34 &34 &34 &38 &38 &38 &38 &42 &42 &42 &42 &42 &42 &42 &42 &\underline{34} &34 &\underline{34} &34 &38 &38 &\underline{38} &38 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &34 &34 &34 &34 &38 &38 &38 &38 &42 &42 &42 &42 &42 &42 &42 &42 &\\
35 &35 &35 &35 &39 &39 &39 &39 &43 &43 &43 &43 &43 &43 &43 &43 &35 &35 &35 &35 &39 &39 &39 &39 &43 &43 &43 &43 &43 &43 &43 &43 &35 &\underline{35} &35 &\underline{35} &39 &39 &39 &\underline{39} &43 &\underline{43} &43 &\underline{43} &43 &43 &43 &43 &35 &35 &35 &35 &39 &39 &39 &39 &43 &43 &43 &43 &43 &43 &43 &43 &\\
\underline{36} &37 &36 &37 &\underline{36} &37 &36 &37 &44 &45 &44 &45 &\underline{44} &45 &44 &45 &36 &37 &36 &37 &36 &37 &36 &37 &44 &45 &44 &45 &44 &45 &44 &45 &\underline{36} &\underline{37} &36 &37 &\underline{36} &\underline{37} &36 &37 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &36 &37 &36 &37 &36 &37 &36 &37 &44 &45 &44 &45 &44 &45 &44 &45 &\\
\underline{37} &37 &37 &37 &\underline{37} &37 &37 &37 &45 &45 &45 &45 &\underline{45} &45 &45 &45 &37 &37 &37 &37 &37 &37 &37 &37 &45 &45 &45 &45 &45 &45 &45 &45 &\underline{37} &\underline{37} &37 &37 &\underline{37} &\underline{37} &37 &37 &45 &45 &45 &45 &\underline{45} &\underline{45} &45 &45 &37 &37 &37 &37 &37 &37 &37 &37 &45 &45 &45 &45 &45 &45 &45 &45 &\\
38 &38 &\underline{38} &38 &38 &38 &\underline{38} &38 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &38 &38 &38 &38 &38 &38 &38 &38 &46 &46 &46 &46 &46 &46 &46 &46 &38 &38 &\underline{38} &38 &38 &38 &\underline{38} &38 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &38 &38 &38 &38 &38 &38 &38 &38 &46 &46 &46 &46 &46 &46 &46 &46 &\\
39 &39 &39 &39 &39 &39 &39 &39 &47 &47 &47 &47 &47 &47 &47 &47 &39 &39 &39 &39 &39 &39 &39 &39 &47 &47 &47 &47 &47 &47 &47 &47 &39 &39 &39 &\underline{39} &39 &39 &39 &\underline{39} &47 &47 &47 &47 &47 &47 &47 &\underline{47} &39 &39 &39 &39 &39 &39 &39 &39 &47 &47 &47 &47 &47 &47 &47 &47 &\\
\underline{40} &41 &\underline{42} &42 &40 &41 &42 &42 &\underline{40} &41 &\underline{42} &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &\underline{40} &\underline{41} &\underline{42} &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &40 &41 &42 &42 &\\
\underline{41} &41 &43 &43 &41 &41 &43 &43 &\underline{41} &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &\underline{41} &\underline{41} &43 &\underline{43} &41 &41 &43 &43 &\underline{41} &\underline{41} &43 &\underline{43} &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &41 &41 &43 &43 &\\
\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &\underline{42} &42 &\underline{42} &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &42 &\\
43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &\underline{43} &43 &\underline{43} &43 &43 &43 &43 &43 &\underline{43} &43 &\underline{43} &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &43 &\\
44 &45 &44 &45 &\underline{44} &45 &44 &45 &44 &45 &44 &45 &\underline{44} &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &44 &45 &44 &45 &\underline{44} &\underline{45} &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &44 &45 &\\
45 &45 &45 &45 &\underline{45} &45 &45 &45 &45 &45 &45 &45 &\underline{45} &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &\underline{45} &\underline{45} &45 &45 &45 &45 &45 &45 &\underline{45} &\underline{45} &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &45 &\\
46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &\underline{46} &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &46 &\\
47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{47} &47 &47 &47 &47 &47 &47 &47 &\underline{47} &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &47 &\\
48 &49 &50 &50 &52 &53 &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &\underline{48} &49 &\underline{50} &50 &\underline{52} &53 &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &\underline{48} &\underline{49} &\underline{50} &50 &\underline{52} &\underline{53} &52 &53 &48 &49 &50 &50 &52 &53 &52 &53 &\\
49 &49 &51 &51 &53 &53 &53 &53 &49 &49 &51 &51 &53 &53 &53 &53 &\underline{49} &49 &51 &51 &\underline{53} &53 &53 &53 &49 &49 &51 &51 &53 &53 &53 &53 &49 &49 &51 &51 &53 &53 &53 &53 &49 &49 &51 &51 &53 &53 &53 &53 &\underline{49} &\underline{49} &51 &\underline{51} &\underline{53} &\underline{53} &53 &53 &49 &49 &51 &51 &53 &53 &53 &53 &\\
50 &50 &50 &50 &54 &54 &54 &54 &50 &50 &50 &50 &54 &54 &54 &54 &\underline{50} &50 &\underline{50} &50 &54 &54 &\underline{54} &54 &50 &50 &50 &50 &54 &54 &54 &54 &50 &50 &50 &50 &54 &54 &54 &54 &50 &50 &50 &50 &54 &54 &54 &54 &\underline{50} &50 &\underline{50} &50 &54 &54 &\underline{54} &54 &50 &50 &50 &50 &54 &54 &54 &54 &\\
51 &51 &51 &51 &55 &55 &55 &55 &51 &51 &51 &51 &55 &55 &55 &55 &51 &51 &51 &51 &55 &55 &55 &55 &51 &51 &51 &51 &55 &55 &55 &55 &51 &51 &51 &51 &55 &55 &55 &55 &51 &51 &51 &51 &55 &55 &55 &55 &51 &\underline{51} &51 &\underline{51} &55 &55 &55 &\underline{55} &51 &51 &51 &51 &55 &55 &55 &55 &\\
52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &\underline{52} &53 &52 &53 &\underline{52} &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &\underline{52} &\underline{53} &52 &53 &\underline{52} &\underline{53} &52 &53 &52 &53 &52 &53 &52 &53 &52 &53 &\\
53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &\underline{53} &53 &53 &53 &\underline{53} &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &\underline{53} &\underline{53} &53 &53 &\underline{53} &\underline{53} &53 &53 &53 &53 &53 &53 &53 &53 &53 &53 &\\
54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &\underline{54} &54 &54 &54 &\underline{54} &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &54 &\underline{54} &54 &54 &54 &\underline{54} &54 &54 &54 &54 &54 &54 &54 &54 &54 &\\
55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &55 &\underline{55} &55 &55 &55 &\underline{55} &55 &55 &55 &55 &55 &55 &55 &55 &\\
56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &\underline{56} &57 &\underline{58} &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &56 &57 &58 &58 &\underline{56} &\underline{57} &\underline{58} &58 &56 &57 &58 &58 &\\
57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &\underline{57} &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &57 &57 &59 &59 &\underline{57} &\underline{57} &59 &\underline{59} &57 &57 &59 &59 &\\
58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &\underline{58} &58 &\underline{58} &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &58 &\underline{58} &58 &\underline{58} &58 &58 &58 &58 &58 &\\
59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &59 &\underline{59} &59 &\underline{59} &59 &59 &59 &59 &\\
60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &\underline{60} &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &60 &61 &\underline{60} &\underline{61} &60 &61 &\\
61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &\underline{61} &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &61 &\underline{61} &\underline{61} &61 &61 &\\
62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &\underline{62} &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &\underline{62} &62 &\\
63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &\underline{63} &\\
\end{smallmatrix}$$
\end{scriptsize}


==> matrices/matrixTEX_L3.tex <==
\begin{scriptsize}
$$\begin{smallmatrix}
\underline{0}  &2  &4  &6  &8  &10 &12 &14 &16 &18 &20 &22 &24 &26 &28 &30 &32 &34 &36 &38 &40 &42 &44 &46 &48 &50 &52 &54 &56 &58 &60 &62 &1  &3  &5  &7  &9  &11 &13 &15 &17 &19 &21 &23 &25 &27 &29 &31 &33 &35 &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &\underline{63} &\\
1  &\underline{3}  &5  &7  &9  &11 &13 &15 &17 &19 &21 &23 &25 &27 &29 &31 &33 &35 &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &63 &33 &\underline{35} &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &63 &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
2  &3  &\underline{6}  &\underline{7}  &10 &11 &14 &15 &18 &19 &22 &23 &26 &27 &30 &31 &34 &35 &38 &39 &42 &43 &46 &47 &50 &51 &54 &55 &58 &59 &62 &63 &3  &3  &7  &7  &11 &11 &15 &15 &19 &19 &23 &23 &27 &27 &31 &31 &35 &35 &39 &39 &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &\underline{63} &\\
3  &3  &\underline{7}  &\underline{7}  &11 &11 &15 &15 &19 &19 &23 &23 &27 &27 &31 &31 &35 &35 &39 &39 &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &63 &35 &35 &\underline{39} &\underline{39} &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &63 &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
4  &6  &6  &7  &\underline{12} &14 &\underline{14} &\underline{15} &20 &22 &22 &23 &28 &30 &30 &31 &36 &38 &38 &39 &44 &46 &46 &47 &52 &54 &54 &55 &60 &62 &62 &63 &5  &7  &7  &7  &13 &15 &15 &15 &21 &23 &23 &23 &29 &31 &31 &31 &37 &39 &39 &39 &45 &47 &47 &47 &53 &55 &55 &55 &61 &63 &63 &\underline{63} &\\
5  &7  &7  &7  &13 &\underline{15} &\underline{15} &\underline{15} &21 &23 &23 &23 &29 &31 &31 &31 &37 &39 &39 &39 &45 &47 &47 &47 &53 &55 &55 &55 &61 &63 &63 &63 &37 &39 &39 &39 &45 &\underline{47} &\underline{47} &\underline{47} &53 &55 &55 &55 &61 &63 &63 &63 &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
6  &7  &6  &7  &\underline{14} &\underline{15} &\underline{14} &\underline{15} &22 &23 &22 &23 &30 &31 &30 &31 &38 &39 &38 &39 &46 &47 &46 &47 &54 &55 &54 &55 &62 &63 &62 &63 &7  &7  &7  &7  &15 &15 &15 &15 &23 &23 &23 &23 &31 &31 &31 &31 &39 &39 &39 &39 &47 &47 &47 &47 &55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &\\
7  &7  &7  &7  &\underline{15} &\underline{15} &\underline{15} &\underline{15} &23 &23 &23 &23 &31 &31 &31 &31 &39 &39 &39 &39 &47 &47 &47 &47 &55 &55 &55 &55 &63 &63 &63 &63 &39 &39 &39 &39 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
8  &10 &12 &14 &12 &14 &14 &15 &\underline{24} &26 &28 &30 &\underline{28} &30 &\underline{30} &\underline{31} &40 &42 &44 &46 &44 &46 &46 &47 &56 &58 &60 &62 &60 &62 &62 &63 &9  &11 &13 &15 &13 &15 &15 &15 &25 &27 &29 &31 &29 &31 &31 &31 &41 &43 &45 &47 &45 &47 &47 &47 &57 &59 &61 &63 &61 &63 &63 &\underline{63} &\\
9  &11 &13 &15 &13 &15 &15 &15 &25 &\underline{27} &29 &31 &29 &\underline{31} &\underline{31} &\underline{31} &41 &43 &45 &47 &45 &47 &47 &47 &57 &59 &61 &63 &61 &63 &63 &63 &41 &43 &45 &47 &45 &47 &47 &47 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
10 &11 &14 &15 &14 &15 &14 &15 &26 &27 &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &42 &43 &46 &47 &46 &47 &46 &47 &58 &59 &62 &63 &62 &63 &62 &63 &11 &11 &15 &15 &15 &15 &15 &15 &27 &27 &31 &31 &31 &31 &31 &31 &43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
11 &11 &15 &15 &15 &15 &15 &15 &27 &27 &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &63 &63 &63 &63 &63 &63 &43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
12 &14 &14 &15 &12 &14 &14 &15 &\underline{28} &30 &\underline{30} &\underline{31} &\underline{28} &30 &\underline{30} &\underline{31} &44 &46 &46 &47 &44 &46 &46 &47 &60 &62 &62 &63 &60 &62 &62 &63 &13 &15 &15 &15 &13 &15 &15 &15 &29 &31 &31 &31 &29 &31 &31 &31 &45 &47 &47 &47 &45 &47 &47 &47 &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &\\
13 &15 &15 &15 &13 &15 &15 &15 &29 &\underline{31} &\underline{31} &\underline{31} &29 &\underline{31} &\underline{31} &\underline{31} &45 &47 &47 &47 &45 &47 &47 &47 &61 &63 &63 &63 &61 &63 &63 &63 &45 &47 &47 &47 &45 &47 &47 &47 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
14 &15 &14 &15 &14 &15 &14 &15 &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &\underline{30} &\underline{31} &46 &47 &46 &47 &46 &47 &46 &47 &62 &63 &62 &63 &62 &63 &62 &63 &15 &15 &15 &15 &15 &15 &15 &15 &31 &31 &31 &31 &31 &31 &31 &31 &47 &47 &47 &47 &47 &47 &47 &47 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
15 &15 &15 &15 &15 &15 &15 &15 &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &\underline{31} &47 &47 &47 &47 &47 &47 &47 &47 &63 &63 &63 &63 &63 &63 &63 &63 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
16 &18 &20 &22 &24 &26 &28 &30 &24 &26 &28 &30 &28 &30 &30 &31 &\underline{48} &50 &52 &54 &56 &58 &60 &62 &\underline{56} &58 &60 &62 &\underline{60} &62 &\underline{62} &\underline{63} &17 &19 &21 &23 &25 &27 &29 &31 &25 &27 &29 &31 &29 &31 &31 &31 &49 &51 &53 &55 &57 &59 &61 &63 &57 &59 &61 &63 &61 &63 &63 &\underline{63} &\\
17 &19 &21 &23 &25 &27 &29 &31 &25 &27 &29 &31 &29 &31 &31 &31 &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
18 &19 &22 &23 &26 &27 &30 &31 &26 &27 &30 &31 &30 &31 &30 &31 &50 &51 &\underline{54} &\underline{55} &58 &59 &62 &63 &58 &59 &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &19 &19 &23 &23 &27 &27 &31 &31 &27 &27 &31 &31 &31 &31 &31 &31 &51 &51 &55 &\underline{55} &59 &59 &63 &63 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
19 &19 &23 &23 &27 &27 &31 &31 &27 &27 &31 &31 &31 &31 &31 &31 &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
20 &22 &22 &23 &28 &30 &30 &31 &28 &30 &30 &31 &28 &30 &30 &31 &52 &54 &54 &55 &\underline{60} &62 &\underline{62} &\underline{63} &\underline{60} &62 &\underline{62} &\underline{63} &\underline{60} &62 &\underline{62} &\underline{63} &21 &23 &23 &23 &29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &53 &55 &55 &55 &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &\\
21 &23 &23 &23 &29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
22 &23 &22 &23 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &54 &55 &54 &55 &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &23 &23 &23 &23 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
23 &23 &23 &23 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
24 &26 &28 &30 &28 &30 &30 &31 &24 &26 &28 &30 &28 &30 &30 &31 &\underline{56} &58 &60 &62 &\underline{60} &62 &\underline{62} &\underline{63} &\underline{56} &58 &60 &62 &\underline{60} &62 &\underline{62} &\underline{63} &25 &27 &29 &31 &29 &31 &31 &31 &25 &27 &29 &31 &29 &31 &31 &31 &57 &59 &61 &63 &61 &63 &63 &\underline{63} &57 &59 &61 &63 &61 &63 &63 &\underline{63} &\\
25 &27 &29 &31 &29 &31 &31 &31 &25 &27 &29 &31 &29 &31 &31 &31 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
26 &27 &30 &31 &30 &31 &30 &31 &26 &27 &30 &31 &30 &31 &30 &31 &58 &59 &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &58 &59 &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &27 &27 &31 &31 &31 &31 &31 &31 &27 &27 &31 &31 &31 &31 &31 &31 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
27 &27 &31 &31 &31 &31 &31 &31 &27 &27 &31 &31 &31 &31 &31 &31 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
28 &30 &30 &31 &28 &30 &30 &31 &28 &30 &30 &31 &28 &30 &30 &31 &\underline{60} &62 &\underline{62} &\underline{63} &\underline{60} &62 &\underline{62} &\underline{63} &\underline{60} &62 &\underline{62} &\underline{63} &\underline{60} &62 &\underline{62} &\underline{63} &29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &61 &63 &63 &\underline{63} &\\
29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &29 &31 &31 &31 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &30 &31 &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &\underline{62} &\underline{63} &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\\
31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
32 &34 &36 &38 &40 &42 &44 &46 &48 &50 &52 &54 &56 &58 &60 &62 &48 &50 &52 &54 &56 &58 &60 &62 &56 &58 &60 &62 &60 &62 &62 &\underline{63} &\underline{33} &35 &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &63 &\underline{49} &51 &53 &55 &57 &59 &61 &63 &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\\
33 &\underline{35} &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &63 &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &33 &\underline{35} &37 &39 &41 &43 &45 &47 &49 &51 &53 &55 &57 &59 &61 &63 &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
34 &35 &38 &\underline{39} &42 &43 &46 &47 &50 &51 &54 &55 &58 &59 &62 &63 &50 &51 &54 &\underline{55} &58 &59 &62 &63 &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &35 &35 &\underline{39} &\underline{39} &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &63 &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
35 &35 &39 &\underline{39} &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &63 &51 &51 &55 &\underline{55} &59 &59 &63 &63 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &35 &35 &\underline{39} &\underline{39} &43 &43 &47 &47 &51 &51 &55 &55 &59 &59 &63 &63 &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
36 &38 &38 &39 &44 &46 &46 &\underline{47} &52 &54 &54 &55 &60 &62 &62 &63 &52 &54 &54 &55 &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &37 &39 &39 &39 &\underline{45} &47 &\underline{47} &\underline{47} &53 &55 &55 &55 &61 &63 &63 &63 &53 &55 &55 &55 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\\
37 &39 &39 &39 &45 &\underline{47} &47 &\underline{47} &53 &55 &55 &55 &61 &63 &63 &63 &53 &55 &55 &55 &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &37 &39 &39 &39 &45 &\underline{47} &\underline{47} &\underline{47} &53 &55 &55 &55 &61 &63 &63 &63 &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
38 &39 &38 &39 &46 &\underline{47} &46 &\underline{47} &54 &55 &54 &55 &62 &63 &62 &63 &54 &55 &54 &55 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &39 &39 &39 &39 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
39 &39 &39 &39 &47 &\underline{47} &47 &\underline{47} &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &39 &39 &39 &39 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
40 &42 &44 &46 &44 &46 &46 &47 &56 &58 &60 &62 &60 &62 &62 &\underline{63} &56 &58 &60 &62 &60 &62 &62 &\underline{63} &56 &58 &60 &62 &60 &62 &62 &\underline{63} &41 &43 &45 &47 &45 &47 &47 &47 &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\\
41 &43 &45 &47 &45 &47 &47 &47 &57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &41 &43 &45 &47 &45 &47 &47 &47 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
42 &43 &46 &47 &46 &47 &46 &47 &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &43 &43 &47 &47 &47 &47 &47 &47 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
44 &46 &46 &47 &44 &46 &46 &47 &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &45 &47 &47 &47 &45 &47 &47 &47 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\\
45 &47 &47 &47 &45 &47 &47 &47 &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &45 &47 &47 &47 &45 &47 &47 &47 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
46 &47 &46 &47 &46 &47 &46 &47 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
47 &47 &47 &47 &47 &47 &47 &47 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
48 &50 &52 &54 &56 &58 &60 &62 &56 &58 &60 &62 &60 &62 &62 &\underline{63} &48 &50 &52 &54 &56 &58 &60 &62 &56 &58 &60 &62 &60 &62 &62 &\underline{63} &\underline{49} &51 &53 &55 &57 &59 &61 &63 &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{49} &51 &53 &55 &57 &59 &61 &63 &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\\
49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &49 &\underline{51} &53 &55 &57 &59 &61 &63 &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
50 &51 &54 &\underline{55} &58 &59 &62 &63 &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &50 &51 &54 &\underline{55} &58 &59 &62 &63 &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
51 &51 &55 &\underline{55} &59 &59 &63 &63 &59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &\underline{55} &\underline{55} &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
52 &54 &54 &55 &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &52 &54 &54 &55 &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &53 &55 &55 &55 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &53 &55 &55 &55 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\\
53 &55 &55 &55 &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &63 &\underline{63} &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &53 &55 &55 &55 &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
54 &55 &54 &55 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &54 &55 &54 &55 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
56 &58 &60 &62 &60 &62 &62 &\underline{63} &56 &58 &60 &62 &60 &62 &62 &\underline{63} &56 &58 &60 &62 &60 &62 &62 &\underline{63} &56 &58 &60 &62 &60 &62 &62 &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\underline{57} &59 &61 &63 &\underline{61} &63 &\underline{63} &\underline{63} &\\
57 &\underline{59} &61 &63 &61 &\underline{63} &63 &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &57 &\underline{59} &61 &63 &61 &\underline{63} &\underline{63} &\underline{63} &\\
58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &58 &59 &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
59 &59 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &60 &62 &62 &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\underline{61} &63 &\underline{63} &\underline{63} &\\
61 &\underline{63} &63 &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &61 &\underline{63} &\underline{63} &\underline{63} &\\
62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &62 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
\end{smallmatrix}$$
\end{scriptsize}


==> matrices/matrixTEX_L4.tex <==
\begin{scriptsize}
$$\begin{smallmatrix}
\underline{0}  &3  &6  &6  &12 &15 &12 &15 &24 &27 &30 &30 &24 &27 &30 &30 &48 &51 &54 &54 &60 &63 &60 &63 &48 &51 &54 &54 &60 &63 &60 &63 &33 &35 &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &63 &63 &33 &35 &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &63 &\underline{63} &\\
1  &\underline{3}  &7  &7  &13 &15 &13 &15 &25 &27 &31 &31 &25 &27 &31 &31 &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &63 &1  &3  &7  &7  &13 &15 &13 &15 &25 &27 &31 &31 &25 &27 &31 &31 &49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &\\
2  &2  &\underline{6}  &6  &14 &14 &14 &14 &26 &26 &30 &30 &26 &26 &30 &30 &50 &50 &54 &54 &62 &62 &62 &62 &50 &50 &54 &54 &62 &62 &62 &62 &35 &35 &39 &\underline{39} &47 &47 &47 &47 &59 &59 &63 &63 &59 &59 &63 &63 &35 &35 &39 &39 &47 &47 &47 &47 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &\\
3  &3  &7  &\underline{7}  &15 &15 &15 &15 &27 &27 &31 &31 &27 &27 &31 &31 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &63 &63 &3  &3  &7  &7  &15 &15 &15 &15 &27 &27 &31 &31 &27 &27 &31 &31 &51 &51 &55 &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &\\
4  &7  &4  &7  &\underline{12} &15 &12 &\underline{15} &28 &31 &28 &31 &28 &31 &28 &31 &52 &55 &52 &55 &60 &63 &60 &63 &52 &55 &52 &55 &60 &63 &60 &63 &37 &39 &37 &39 &45 &47 &45 &\underline{47} &61 &63 &61 &63 &61 &63 &61 &63 &37 &39 &37 &39 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &\underline{63} &\\
5  &7  &5  &7  &13 &\underline{15} &13 &\underline{15} &29 &31 &29 &31 &29 &31 &29 &31 &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &63 &61 &63 &5  &7  &5  &7  &13 &15 &13 &15 &29 &31 &29 &31 &29 &31 &29 &31 &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &\\
6  &6  &6  &6  &14 &14 &\underline{14} &14 &30 &30 &30 &30 &30 &30 &30 &30 &54 &54 &54 &54 &62 &62 &62 &62 &54 &54 &54 &54 &62 &62 &62 &62 &39 &39 &39 &39 &47 &47 &47 &\underline{47} &63 &63 &63 &63 &63 &63 &63 &63 &39 &39 &39 &39 &47 &47 &47 &47 &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &\\
7  &7  &7  &7  &\underline{15} &\underline{15} &15 &\underline{15} &31 &31 &31 &31 &31 &31 &31 &31 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &63 &63 &7  &7  &7  &7  &15 &15 &15 &15 &31 &31 &31 &31 &31 &31 &31 &31 &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &\\
8  &11 &14 &14 &8  &11 &14 &14 &\underline{24} &27 &30 &30 &24 &27 &\underline{30} &30 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &41 &43 &47 &47 &41 &43 &47 &47 &57 &59 &63 &63 &57 &59 &63 &\underline{63} &41 &43 &47 &47 &41 &43 &47 &47 &57 &59 &63 &63 &57 &59 &63 &\underline{63} &\\
9  &11 &15 &15 &9  &11 &15 &15 &25 &\underline{27} &31 &31 &25 &27 &31 &\underline{31} &57 &59 &63 &63 &57 &59 &63 &63 &57 &59 &63 &63 &57 &59 &63 &63 &9  &11 &15 &15 &9  &11 &15 &15 &25 &27 &31 &31 &25 &27 &31 &31 &57 &59 &63 &63 &57 &59 &63 &63 &57 &\underline{59} &63 &63 &57 &59 &63 &\underline{63} &\\
10 &10 &14 &14 &10 &10 &14 &14 &26 &26 &\underline{30} &30 &26 &26 &\underline{30} &30 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &\\
11 &11 &15 &15 &11 &11 &15 &15 &27 &27 &31 &\underline{31} &27 &27 &31 &\underline{31} &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &63 &11 &11 &15 &15 &11 &11 &15 &15 &27 &27 &31 &31 &27 &27 &31 &31 &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &\\
12 &15 &12 &15 &12 &15 &12 &15 &28 &31 &28 &31 &\underline{28} &31 &28 &\underline{31} &60 &63 &60 &63 &60 &63 &60 &63 &60 &63 &60 &63 &60 &63 &60 &63 &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &\underline{63} &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &\underline{63} &\\
13 &15 &13 &15 &13 &15 &13 &15 &29 &31 &29 &31 &29 &\underline{31} &29 &\underline{31} &61 &63 &61 &63 &61 &63 &61 &63 &61 &63 &61 &63 &61 &63 &61 &63 &13 &15 &13 &15 &13 &15 &13 &15 &29 &31 &29 &31 &29 &31 &29 &31 &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &\\
14 &14 &14 &14 &14 &14 &14 &14 &\underline{30} &30 &\underline{30} &30 &30 &30 &\underline{30} &30 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &47 &47 &47 &47 &47 &47 &47 &47 &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &\\
15 &15 &15 &15 &15 &15 &15 &15 &31 &\underline{31} &31 &\underline{31} &\underline{31} &\underline{31} &31 &\underline{31} &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &63 &15 &15 &15 &15 &15 &15 &15 &15 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{63} &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &\\
16 &19 &22 &22 &28 &31 &28 &31 &16 &19 &22 &22 &28 &31 &28 &31 &\underline{48} &51 &54 &54 &60 &63 &60 &63 &48 &51 &54 &54 &\underline{60} &63 &60 &\underline{63} &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &\underline{63} &\\
17 &19 &23 &23 &29 &31 &29 &31 &17 &19 &23 &23 &29 &31 &29 &31 &49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &17 &19 &23 &23 &29 &31 &29 &31 &17 &19 &23 &23 &29 &31 &29 &31 &49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &\\
18 &18 &22 &22 &30 &30 &30 &30 &18 &18 &22 &22 &30 &30 &30 &30 &50 &50 &\underline{54} &54 &62 &62 &62 &62 &50 &50 &54 &54 &62 &62 &\underline{62} &62 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &55 &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &63 &\underline{63} &\\
19 &19 &23 &23 &31 &31 &31 &31 &19 &19 &23 &23 &31 &31 &31 &31 &51 &51 &55 &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &19 &19 &23 &23 &31 &31 &31 &31 &19 &19 &23 &23 &31 &31 &31 &31 &51 &51 &55 &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &\\
20 &23 &20 &23 &28 &31 &28 &31 &20 &23 &20 &23 &28 &31 &28 &31 &52 &55 &52 &55 &\underline{60} &63 &60 &\underline{63} &52 &55 &52 &55 &\underline{60} &63 &60 &\underline{63} &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &63 &61 &\underline{63} &53 &55 &53 &55 &61 &63 &61 &\underline{63} &\\
21 &23 &21 &23 &29 &31 &29 &31 &21 &23 &21 &23 &29 &31 &29 &31 &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &21 &23 &21 &23 &29 &31 &29 &31 &21 &23 &21 &23 &29 &31 &29 &31 &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &\\
22 &22 &22 &22 &30 &30 &30 &30 &22 &22 &22 &22 &30 &30 &30 &30 &54 &54 &54 &54 &62 &62 &\underline{62} &62 &54 &54 &54 &54 &62 &62 &\underline{62} &62 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &63 &\underline{63} &55 &55 &55 &55 &63 &63 &63 &\underline{63} &\\
23 &23 &23 &23 &31 &31 &31 &31 &23 &23 &23 &23 &31 &31 &31 &31 &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &23 &23 &23 &23 &31 &31 &31 &31 &23 &23 &23 &23 &31 &31 &31 &31 &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &63 &\underline{63} &\\
24 &27 &30 &30 &24 &27 &30 &30 &24 &27 &30 &30 &24 &27 &30 &30 &56 &59 &62 &62 &56 &59 &62 &62 &\underline{56} &59 &62 &62 &56 &59 &\underline{62} &62 &57 &59 &63 &63 &57 &59 &63 &\underline{63} &57 &59 &63 &63 &57 &59 &63 &\underline{63} &57 &59 &63 &63 &57 &59 &63 &63 &57 &59 &63 &63 &57 &59 &63 &\underline{63} &\\
25 &27 &31 &31 &25 &27 &31 &31 &25 &27 &31 &31 &25 &27 &31 &31 &57 &59 &63 &63 &57 &59 &63 &63 &57 &\underline{59} &63 &63 &57 &59 &63 &\underline{63} &25 &27 &31 &31 &25 &27 &31 &31 &25 &27 &31 &31 &25 &27 &31 &31 &57 &59 &63 &63 &57 &59 &63 &63 &57 &\underline{59} &63 &63 &57 &59 &63 &\underline{63} &\\
26 &26 &30 &30 &26 &26 &30 &30 &26 &26 &30 &30 &26 &26 &30 &30 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &\underline{62} &62 &58 &58 &\underline{62} &62 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &\\
27 &27 &31 &31 &27 &27 &31 &31 &27 &27 &31 &31 &27 &27 &31 &31 &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &27 &27 &31 &31 &27 &27 &31 &31 &27 &27 &31 &31 &27 &27 &31 &31 &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &63 &\underline{63} &59 &59 &63 &\underline{63} &\\
28 &31 &28 &31 &28 &31 &28 &31 &28 &31 &28 &31 &28 &31 &28 &31 &\underline{60} &63 &60 &\underline{63} &\underline{60} &63 &60 &\underline{63} &60 &63 &60 &63 &\underline{60} &63 &60 &\underline{63} &61 &63 &61 &63 &61 &63 &61 &\underline{63} &61 &63 &61 &63 &61 &63 &61 &\underline{63} &61 &63 &61 &\underline{63} &61 &63 &61 &\underline{63} &61 &63 &61 &63 &61 &63 &61 &\underline{63} &\\
29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &29 &31 &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &\\
30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &30 &62 &62 &\underline{62} &62 &62 &62 &\underline{62} &62 &\underline{62} &62 &\underline{62} &62 &62 &62 &\underline{62} &62 &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &63 &63 &63 &\underline{63} &63 &63 &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &63 &63 &\underline{63} &\\
31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{63} &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &31 &\underline{63} &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &\underline{63} &\underline{63} &63 &\underline{63} &\\
32 &35 &38 &38 &44 &47 &44 &47 &56 &59 &62 &62 &56 &59 &62 &62 &32 &35 &38 &38 &44 &47 &44 &47 &56 &59 &62 &62 &56 &59 &62 &62 &\underline{33} &35 &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &63 &63 &33 &35 &39 &39 &45 &47 &45 &47 &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
33 &35 &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &63 &63 &33 &35 &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &\underline{63} &63 &33 &\underline{35} &39 &39 &45 &47 &45 &47 &57 &59 &63 &63 &57 &59 &63 &63 &33 &35 &39 &39 &45 &47 &45 &47 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
34 &34 &38 &38 &46 &46 &46 &46 &58 &58 &62 &62 &58 &58 &62 &62 &34 &34 &38 &38 &46 &46 &46 &46 &58 &58 &62 &62 &58 &58 &62 &62 &35 &35 &\underline{39} &\underline{39} &47 &47 &47 &47 &59 &59 &63 &63 &59 &59 &63 &63 &35 &35 &39 &39 &47 &47 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
35 &35 &\underline{39} &39 &47 &47 &47 &47 &59 &59 &63 &63 &59 &59 &63 &63 &35 &35 &39 &39 &47 &47 &47 &47 &59 &59 &\underline{63} &63 &59 &59 &\underline{63} &63 &35 &35 &\underline{39} &\underline{39} &47 &47 &47 &47 &59 &59 &63 &63 &59 &59 &63 &63 &35 &35 &39 &39 &47 &47 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
36 &39 &36 &39 &44 &47 &44 &47 &60 &63 &60 &63 &60 &63 &60 &63 &36 &39 &36 &39 &44 &47 &44 &47 &60 &63 &60 &63 &60 &63 &60 &63 &37 &39 &37 &39 &\underline{45} &47 &45 &\underline{47} &61 &63 &61 &63 &61 &63 &61 &63 &37 &39 &37 &39 &45 &47 &45 &47 &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &\\
37 &39 &37 &39 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &63 &37 &39 &37 &39 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &63 &37 &39 &37 &39 &45 &\underline{47} &45 &\underline{47} &61 &63 &61 &63 &61 &63 &61 &63 &37 &39 &37 &39 &45 &47 &45 &47 &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &\\
38 &38 &38 &38 &46 &46 &46 &46 &62 &62 &62 &62 &62 &62 &62 &62 &38 &38 &38 &38 &46 &46 &46 &46 &62 &62 &62 &62 &62 &62 &62 &62 &39 &39 &39 &39 &47 &47 &\underline{47} &\underline{47} &63 &63 &63 &63 &63 &63 &63 &63 &39 &39 &39 &39 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &\\
39 &39 &39 &39 &\underline{47} &47 &\underline{47} &47 &63 &63 &63 &63 &63 &63 &63 &63 &39 &39 &39 &39 &47 &47 &47 &47 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &39 &39 &39 &39 &\underline{47} &\underline{47} &\underline{47} &\underline{47} &63 &63 &63 &63 &63 &63 &63 &63 &39 &39 &39 &39 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
40 &43 &46 &46 &40 &43 &46 &46 &56 &59 &62 &62 &56 &59 &62 &62 &40 &43 &46 &46 &40 &43 &46 &46 &56 &59 &62 &62 &56 &59 &62 &62 &41 &43 &47 &47 &41 &43 &47 &47 &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &41 &43 &47 &47 &41 &43 &47 &47 &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
41 &43 &47 &47 &41 &43 &47 &47 &57 &59 &63 &63 &57 &59 &\underline{63} &63 &41 &43 &47 &47 &41 &43 &47 &47 &57 &59 &63 &63 &57 &59 &\underline{63} &63 &41 &43 &47 &47 &41 &43 &47 &47 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &41 &43 &47 &47 &41 &43 &47 &47 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
42 &42 &46 &46 &42 &42 &46 &46 &58 &58 &62 &62 &58 &58 &62 &62 &42 &42 &46 &46 &42 &42 &46 &46 &58 &58 &62 &62 &58 &58 &62 &62 &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &63 &59 &59 &\underline{63} &63 &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &63 &59 &59 &\underline{63} &63 &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &43 &43 &47 &47 &43 &43 &47 &47 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
44 &47 &44 &47 &44 &47 &44 &47 &60 &63 &60 &63 &60 &63 &60 &63 &44 &47 &44 &47 &44 &47 &44 &47 &60 &63 &60 &63 &60 &63 &60 &63 &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &\\
45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &63 &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &63 &61 &63 &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &45 &47 &45 &47 &45 &47 &45 &47 &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &\\
46 &46 &46 &46 &46 &46 &46 &46 &62 &62 &62 &62 &62 &62 &62 &62 &46 &46 &46 &46 &46 &46 &46 &46 &62 &62 &62 &62 &62 &62 &62 &62 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &\\
47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &\underline{63} &63 &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &47 &47 &47 &47 &47 &47 &47 &47 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
48 &51 &54 &54 &60 &63 &60 &63 &48 &51 &54 &54 &60 &63 &60 &\underline{63} &48 &51 &54 &54 &60 &63 &60 &63 &48 &51 &54 &54 &60 &63 &60 &\underline{63} &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &63 &\underline{49} &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &\underline{61} &63 &61 &\underline{63} &\\
49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &49 &51 &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &63 &61 &63 &49 &\underline{51} &55 &55 &61 &63 &61 &63 &49 &51 &55 &55 &61 &\underline{63} &61 &\underline{63} &\\
50 &50 &54 &54 &62 &62 &62 &62 &50 &50 &54 &54 &62 &62 &62 &62 &50 &50 &54 &54 &62 &62 &62 &62 &50 &50 &54 &54 &62 &62 &62 &62 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &\underline{55} &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &\underline{63} &\underline{63} &\\
51 &51 &55 &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &63 &\underline{63} &63 &\underline{63} &51 &51 &\underline{55} &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &55 &55 &63 &63 &63 &63 &51 &51 &\underline{55} &\underline{55} &63 &63 &63 &63 &51 &51 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
52 &55 &52 &55 &60 &63 &60 &\underline{63} &52 &55 &52 &55 &60 &63 &60 &\underline{63} &52 &55 &52 &55 &60 &63 &60 &\underline{63} &52 &55 &52 &55 &60 &63 &60 &\underline{63} &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &\underline{61} &63 &61 &\underline{63} &53 &55 &53 &55 &\underline{61} &63 &61 &\underline{63} &\\
53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &63 &61 &63 &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &53 &55 &53 &55 &61 &\underline{63} &61 &\underline{63} &\\
54 &54 &54 &54 &62 &62 &62 &62 &54 &54 &54 &54 &62 &62 &62 &62 &54 &54 &54 &54 &62 &62 &62 &62 &54 &54 &54 &54 &62 &62 &62 &62 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &\underline{63} &\underline{63} &55 &55 &55 &55 &63 &63 &\underline{63} &\underline{63} &\\
55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &63 &\underline{63} &63 &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &63 &63 &63 &63 &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &55 &55 &55 &55 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &56 &59 &62 &62 &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &57 &59 &63 &63 &57 &59 &63 &63 &\underline{57} &59 &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
57 &59 &63 &63 &57 &59 &\underline{63} &63 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &57 &59 &63 &63 &57 &59 &63 &63 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &57 &59 &63 &63 &57 &59 &63 &63 &57 &\underline{59} &63 &63 &57 &59 &\underline{63} &\underline{63} &\\
58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &58 &58 &62 &62 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
59 &59 &\underline{63} &63 &59 &59 &\underline{63} &63 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &59 &59 &63 &63 &59 &59 &63 &63 &59 &59 &\underline{63} &\underline{63} &59 &59 &\underline{63} &\underline{63} &\\
60 &63 &60 &\underline{63} &60 &63 &60 &\underline{63} &60 &63 &60 &63 &60 &63 &60 &\underline{63} &60 &63 &60 &\underline{63} &60 &63 &60 &\underline{63} &60 &63 &60 &63 &60 &63 &60 &\underline{63} &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &\underline{61} &63 &61 &\underline{63} &\underline{61} &63 &61 &\underline{63} &61 &63 &61 &63 &\underline{61} &63 &61 &\underline{63} &\\
61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &\underline{63} &61 &63 &61 &63 &61 &\underline{63} &61 &\underline{63} &\\
62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &62 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &63 &63 &\underline{63} &\underline{63} &\\
\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\underline{63} &\\
\end{smallmatrix}$$
\end{scriptsize}


==> two-eater-coding/1076.tex <==
\begin{picture}(200.0,75.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(4.0,67.5){\circle*{1.}}
\put(12.0,67.5){\circle*{1.}}
\put(20.0,67.5){\circle*{1.}}
\put(28.0,67.5){\circle*{1.}}
\put(36.0,67.5){\circle*{1.}}
\put(44.0,67.5){\circle*{1.}}
\put(52.0,67.5){\circle*{1.}}
\put(60.0,67.5){\circle*{1.}}
\put(68.0,67.5){\circle*{1.}}
\put(76.0,67.5){\circle*{1.}}
\put(84.0,67.5){\circle*{1.}}
\put(92.0,67.5){\circle*{1.}}
\put(100.0,67.5){\circle*{1.}}
\put(108.0,67.5){\circle*{1.}}
\put(116.0,67.5){\circle*{1.}}
\put(124.0,67.5){\circle*{1.}}
\put(132.0,67.5){\circle*{1.}}
\put(140.0,67.5){\circle*{1.}}
\put(148.0,67.5){\circle*{1.}}
\put(156.0,67.5){\circle*{1.}}
\put(164.0,67.5){\circle*{1.}}
\put(172.0,67.5){\circle*{1.}}
\put(180.0,67.5){\circle*{1.}}
\put(188.0,67.5){\circle*{1.}}
\put(196.0,67.5){\circle*{1.}}
\put(8.0,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(24.0,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(40.0,60.0){\circle*{1.}}
\put(48.0,60.0){\circle*{1.}}
\put(56.0,60.0){\circle*{1.}}
\put(64.0,60.0){\circle*{1.}}
\put(72.0,60.0){\circle*{1.}}
\put(80.0,60.0){\circle*{1.}}
\put(88.0,60.0){\circle*{1.}}
\put(96.0,60.0){\circle*{1.}}
\put(104.0,60.0){\circle*{1.}}
\put(112.0,60.0){\circle*{1.}}
\put(120.0,60.0){\circle*{1.}}
\put(128.0,60.0){\circle*{1.}}
\put(136.0,60.0){\circle*{1.}}
\put(144.0,60.0){\circle*{1.}}
\put(152.0,60.0){\circle*{1.}}
\put(160.0,60.0){\circle*{1.}}
\put(168.0,60.0){\circle*{1.}}
\put(176.0,60.0){\circle*{1.}}
\put(184.0,60.0){\circle*{1.}}
\put(192.0,60.0){\circle*{1.}}
\put(200.0,60.0){\circle*{1.}}
\put(4.0,52.5){\circle*{1.}}
\put(12.0,52.5){\circle*{1.}}
\put(20.0,52.5){\circle{7.5}}
\put(28.0,52.5){\circle{7.5}}
\put(36.0,52.5){\circle{7.5}}
\put(44.0,52.5){\circle*{1.}}
\put(52.0,52.5){\circle{7.5}}
\put(60.0,52.5){\circle{7.5}}
\put(68.0,52.5){\circle*{1.}}
\put(76.0,52.5){\circle*{1.}}
\put(84.0,52.5){\circle*{1.}}
\put(92.0,52.5){\circle*{1.}}
\put(100.0,52.5){\circle*{1.}}
\put(108.0,52.5){\circle*{1.}}
\put(116.0,52.5){\circle{7.5}}
\put(124.0,52.5){\circle{7.5}}
\put(132.0,52.5){\circle*{1.}}
\put(140.0,52.5){\circle*{1.}}
\put(148.0,52.5){\circle{7.5}}
\put(156.0,52.5){\circle{7.5}}
\put(164.0,52.5){\circle*{1.}}
\put(172.0,52.5){\circle*{1.}}
\put(180.0,52.5){\circle*{1.}}
\put(188.0,52.5){\circle*{1.}}
\put(196.0,52.5){\circle*{1.}}
\put(8.0,45.0){\circle*{1.}}
\put(16.0,45.0){\circle{7.5}}
\put(24.0,45.0){\circle*{7.0}}
\put(32.0,45.0){\circle*{7.0}}
\put(40.0,45.0){\circle{7.5}}
\put(48.0,45.0){\circle{7.5}}
\put(56.0,45.0){\circle*{7.0}}
\put(64.0,45.0){\circle*{7.0}}
\put(72.0,45.0){\circle{7.5}}
\put(80.0,45.0){\circle*{1.}}
\put(88.0,45.0){\circle*{1.}}
\put(96.0,45.0){\circle*{1.}}
\put(104.0,45.0){\circle{7.5}}
\put(112.0,45.0){\circle*{7.0}}
\put(120.0,45.0){\circle*{7.0}}
\put(128.0,45.0){\circle{7.5}}
\put(136.0,45.0){\circle{7.5}}
\put(144.0,45.0){\circle*{7.0}}
\put(152.0,45.0){\circle*{7.0}}
\put(160.0,45.0){\circle{7.5}}
\put(168.0,45.0){\circle*{1.}}
\put(176.0,45.0){\circle*{1.}}
\put(184.0,45.0){\circle*{1.}}
\put(192.0,45.0){\circle*{1.}}
\put(200.0,45.0){\circle*{1.}}
\put(4.0,37.5){\circle*{1.}}
\put(12.0,37.5){\circle*{1.}}
\put(20.0,37.5){\circle*{7.0}}
\put(28.0,37.5){\circle{7.5}}
\put(36.0,37.5){\circle*{7.0}}
\put(44.0,37.5){\circle{7.5}}
\put(52.0,37.5){\circle*{7.0}}
\put(60.0,37.5){\circle{7.5}}
\put(68.0,37.5){\circle*{7.0}}
\put(76.0,37.5){\circle*{1.}}
\put(84.0,37.5){\circle*{1.}}
\put(92.0,37.5){\circle*{1.}}
\put(100.0,37.5){\circle*{1.}}
\put(108.0,37.5){\circle*{7.0}}
\put(116.0,37.5){\circle{7.5}}
\put(124.0,37.5){\circle*{7.0}}
\put(132.0,37.5){\circle{7.5}}
\put(140.0,37.5){\circle*{7.0}}
\put(148.0,37.5){\circle{7.5}}
\put(156.0,37.5){\circle*{7.0}}
\put(164.0,37.5){\circle*{1.}}
\put(172.0,37.5){\circle*{1.}}
\put(180.0,37.5){\circle*{1.}}
\put(188.0,37.5){\circle*{1.}}
\put(196.0,37.5){\circle*{1.}}
\put(8.0,30.0){\circle*{1.}}
\put(16.0,30.0){\circle{7.5}}
\put(24.0,30.0){\circle*{7.0}}
\put(32.0,30.0){\circle*{7.0}}
\put(40.0,30.0){\circle{7.5}}
\put(48.0,30.0){\circle{7.5}}
\put(56.0,30.0){\circle*{7.0}}
\put(64.0,30.0){\circle*{7.0}}
\put(72.0,30.0){\circle{7.5}}
\put(80.0,30.0){\circle*{1.}}
\put(88.0,30.0){\circle*{1.}}
\put(96.0,30.0){\circle*{1.}}
\put(104.0,30.0){\circle{7.5}}
\put(112.0,30.0){\circle*{7.0}}
\put(120.0,30.0){\circle*{7.0}}
\put(128.0,30.0){\circle{7.5}}
\put(136.0,30.0){\circle{7.5}}
\put(144.0,30.0){\circle*{7.0}}
\put(152.0,30.0){\circle*{7.0}}
\put(160.0,30.0){\circle{7.5}}
\put(168.0,30.0){\circle*{1.}}
\put(176.0,30.0){\circle*{1.}}
\put(184.0,30.0){\circle*{1.}}
\put(192.0,30.0){\circle*{1.}}
\put(200.0,30.0){\circle*{1.}}
\put(4.0,22.5){\circle*{1.}}
\put(12.0,22.5){\circle*{1.}}
\put(20.0,22.5){\circle*{1.}}
\put(28.0,22.5){\circle{7.5}}
\put(36.0,22.5){\circle*{1.}}
\put(44.0,22.5){\circle*{1.}}
\put(52.0,22.5){\circle*{1.}}
\put(60.0,22.5){\circle{7.5}}
\put(68.0,22.5){\circle*{1.}}
\put(76.0,22.5){\circle*{1.}}
\put(84.0,22.5){\circle*{1.}}
\put(92.0,22.5){\circle*{1.}}
\put(100.0,22.5){\circle*{1.}}
\put(108.0,22.5){\circle*{1.}}
\put(116.0,22.5){\circle{7.5}}
\put(124.0,22.5){\circle*{1.}}
\put(132.0,22.5){\circle*{1.}}
\put(140.0,22.5){\circle*{1.}}
\put(148.0,22.5){\circle{7.5}}
\put(156.0,22.5){\circle*{1.}}
\put(164.0,22.5){\circle*{1.}}
\put(172.0,22.5){\circle*{1.}}
\put(180.0,22.5){\circle*{1.}}
\put(188.0,22.5){\circle*{1.}}
\put(196.0,22.5){\circle*{1.}}
\put(8.0,15.0){\circle*{1.}}
\put(16.0,15.0){\circle*{1.}}
\put(24.0,15.0){\circle*{1.}}
\put(32.0,15.0){\circle*{1.}}
\put(40.0,15.0){\circle*{1.}}
\put(48.0,15.0){\circle*{1.}}
\put(56.0,15.0){\circle*{1.}}
\put(64.0,15.0){\circle*{1.}}
\put(72.0,15.0){\circle*{1.}}
\put(80.0,15.0){\circle*{1.}}
\put(88.0,15.0){\circle*{1.}}
\put(96.0,15.0){\circle*{1.}}
\put(104.0,15.0){\circle*{1.}}
\put(112.0,15.0){\circle*{1.}}
\put(120.0,15.0){\circle*{1.}}
\put(128.0,15.0){\circle*{1.}}
\put(136.0,15.0){\circle*{1.}}
\put(144.0,15.0){\circle*{1.}}
\put(152.0,15.0){\circle*{1.}}
\put(160.0,15.0){\circle*{1.}}
\put(168.0,15.0){\circle*{1.}}
\put(176.0,15.0){\circle*{1.}}
\put(184.0,15.0){\circle*{1.}}
\put(192.0,15.0){\circle*{1.}}
\put(200.0,15.0){\circle*{1.}}
\put(4.0,7.5){\circle*{1.}}
\put(12.0,7.5){\circle*{1.}}
\put(20.0,7.5){\circle*{1.}}
\put(28.0,7.5){\circle*{1.}}
\put(36.0,7.5){\circle*{1.}}
\put(44.0,7.5){\circle*{1.}}
\put(52.0,7.5){\circle*{1.}}
\put(60.0,7.5){\circle*{1.}}
\put(68.0,7.5){\circle*{1.}}
\put(76.0,7.5){\circle*{1.}}
\put(84.0,7.5){\circle*{1.}}
\put(92.0,7.5){\circle*{1.}}
\put(100.0,7.5){\circle*{1.}}
\put(108.0,7.5){\circle*{1.}}
\put(116.0,7.5){\circle*{1.}}
\put(124.0,7.5){\circle*{1.}}
\put(132.0,7.5){\circle*{1.}}
\put(140.0,7.5){\circle*{1.}}
\put(148.0,7.5){\circle*{1.}}
\put(156.0,7.5){\circle*{1.}}
\put(164.0,7.5){\circle*{1.}}
\put(172.0,7.5){\circle*{1.}}
\put(180.0,7.5){\circle*{1.}}
\put(188.0,7.5){\circle*{1.}}
\put(196.0,7.5){\circle*{1.}}
\put(8.0,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(24.0,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\put(40.0,0.0){\circle*{1.}}
\put(48.0,0.0){\circle*{1.}}
\put(56.0,0.0){\circle*{1.}}
\put(64.0,0.0){\circle*{1.}}
\put(72.0,0.0){\circle*{1.}}
\put(80.0,0.0){\circle*{1.}}
\put(88.0,0.0){\circle*{1.}}
\put(96.0,0.0){\circle*{1.}}
\put(104.0,0.0){\circle*{1.}}
\put(112.0,0.0){\circle*{1.}}
\put(120.0,0.0){\circle*{1.}}
\put(128.0,0.0){\circle*{1.}}
\put(136.0,0.0){\circle*{1.}}
\put(144.0,0.0){\circle*{1.}}
\put(152.0,0.0){\circle*{1.}}
\put(160.0,0.0){\circle*{1.}}
\put(168.0,0.0){\circle*{1.}}
\put(176.0,0.0){\circle*{1.}}
\put(184.0,0.0){\circle*{1.}}
\put(192.0,0.0){\circle*{1.}}
\put(200.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}


























































































































































































































































































































































